Unifying Regularisation Methods for Continual Learning

Continual Learning addresses the challenge of learning a number of different tasks sequentially. The goal of maintaining knowledge of earlier tasks without re-accessing them starkly conflicts with standard SGD training for artificial neural networks. An influential method to tackle this problem without storing old data are so-called regularisation approaches. They measure the importance of each parameter for solving a given task and subsequently protect important parameters from large changes. In the literature, three ways to measure parameter importance have been put forward and they have inspired a large body of follow-up work. Here, we present strong theoretical and empirical evidence that these three methods, Elastic Weight Consolidation (EWC), Synaptic Intelligence (SI) and Memory Aware Synapses (MAS), are surprisingly similar and are all linked to the same theoretical quantity. Concretely, we show that, despite stemming from very different motivations, both SI and MAS approximate the square root of the Fisher Information, with the Fisher being the theoretically justified basis of EWC. Moreover, we show that for SI the relation to the Fisher -- and in fact its performance -- is due to a previously unknown bias. On top of uncovering unknown similarities and unifying regularisation approaches, we also demonstrate that our insights enable practical performance improvements for large batch training.

==> ic/sections/00_abs2.tex <==
An influential family of methods to tackle this are so-called regularisation approaches. They measure the importance of each parameter for modelling a given distribution and subsequently protect important parameters from large changes. 
The theoretical underpinnings of two popular members of this family, Synaptic Intelligence (SI) and Memory Aware Synapses (MAS), had previously not been understood. 
Here, we present strong theoretical and empirical evidence that both these measures are approximately equal to the square root of the Fisher Information. 
This makes their relation to theoretically justified bayesian methods explicit and shows how these algorithms and their follow ups all rely on information about the curvature.
For SI, our results rely on exhibiting a previously unnoticed bias and showing that this bias rather than the original objective explains its performance.
Beyond a theoretical unification, we demonstrate how the our insights yield practical performance improvements.

==> ic/sections/04_theory.tex <==
\section{Theory \& Methods}
In this section we describe our theoretical results and design experiments to test our hypotheses,  focussing on Memory Aware Synapses (MAS) in Section \ref{sec:memory} and on Synaptic Intelligence (SI) in Section \ref{sec:synaptic}. The empirical results of our experiments will be presented in Section \ref{sec:experiments}. An overview of different algorithms described here can be found in Table \ref{table:overview}.

\begin{table}[t]
	%\vskip -0.1in
	\caption{\textbf{Summary of Regularisation Methods.} The three algorithms SI, MAS, Fisher (EWC) are the three known algorithms, which have inspired serveral follow ups. The other algorithms are introduced here in order to show that SI and MAS are closely related to Absolute Fisher, which is a natural variant of the Fisher Information.\\
		\textit{Details:}
		Algorithms on the left calculate importance `online' along the parameter trajectory during training. Algorithms on the right calculate importance at the end of training a task by going through (part of) the training set again. Thus, the sum is over timesteps $t$ (left) or datapoints $X$ (right). $N$ is the number of images over which is summed. Note that all the algorithms on the left rescale their final importances as in equation \eqref{eq:rescale}.
		$\Delta(t)= \theta(t+1) - \theta(t)$ refers to the parameter update at time $t$, which depends on both the current task's loss and the auxiliary regularisation loss. Moreover, 
		$(g_t+\sigma_t)$ refers to the stochastic gradient estimate of the current task's loss (where $g_t$ is the full gradient and $\sigma_t$ the noise) given to the optimizer to update parameters. In contrast, $(g_t + \sigma_t')$ refers to an independent stochastic gradient estimate.
		For a datapoint $X$, $\textbf{q}_X$ denotes the predicted label distribution and 
		$g(X,y)$ refers to the gradient of the negative log-likelihood of $(X,y)$.
	 }\label{table:overview}
	\iffalse
	\caption{\textbf{Overview of different algorithms and their importance measures for one task.} 
		Algorithms on the left calculate importance `online' along the parameter trajectory during training. Algorithms on the right calculate importance at the end of training a task by going through (part of) the training set again: The sum is over timesteps $t$ (left) or datapoints $X$ (right). $N$ is the number of images over which is summed. Note that all the algorithms on the left rescale their final importances as in equation \eqref{eq:rescale}.
		In all algorithms $\Delta(t)= \theta(t+1) - \theta(t)$ refers to the parameter update at time $t$, which depends on both the current task's loss and the regularisation loss. Moreover, 
		$(g_t+\sigma_t)$ refers to the stochastic gradient estimate of the current task's loss (where $g_t$ is the full gradient and $\sigma_t$ the noise) given to the optimizer (together with the regularisation loss) to calculate the parameter update. In contrast, $(g_t + \sigma_t')$ refers to an independent stochastic gradient estimate of the current task loss.
		For a datapoint $X$, $\textbf{q}_X$ denotes the predicted label distribution and 
		$g(X,y)$ refers to the gradient of the negative log-likelihood of $(X,y)$. }
	\fi
	%\vskip -0.5in
	\centering
	\begin{small}
		\begin{tabular}{ll|c|ll}
			\toprule
			\textbf{Name}  & \makecell{\textbf{Paramater} \\ \textbf{importance } $\mathbf{\omega(\cdot)}$}  &&\textbf{Name}  & \makecell{\textbf{Paramater} \\ \textbf{importance } $\mathbf{\omega(\cdot)}$}
			%&\makecell{\textbf{Normalisation} \\ $\omega(\cdot) \leftarrow \omega(\cdot) / (l^2+\epsilon )$ } 
			\\ \midrule
			SI &  $\displaystyle\sum_{t}^{} (g_t+\sigma_t)\Delta(t)$ && Fisher  & $\displaystyle\frac1N\sum_X \EE_{y\sim \textbf{q}_X}\left[g(X,y)^2 \right] $ %&$\surd$ 
			\\
			%\midrule
			SIU (SI-Unbiased)  & $\displaystyle\sum_t (g_t+\sigma_t')\Delta(t)$ && AF (Absolute Fisher)  & $\displaystyle\frac1N\sum_X \EE_{y\sim \textbf{q}_X}\left[|g(X,y)| \right] $
			%&$\surd$
			\\
			%\midrule
			SIB (SI Bias-only)&  $\displaystyle\sum_t (\sigma_t- \sigma_t')\Delta(t)$  && MAS & $\displaystyle\frac1N\sum_X \left|\frac{\partial ||\textbf{q}_X||^2}{\partial \theta}\right| $
			%&$\surd$ 
			\\
			%	\midrule					
			OnAF (Online AF)  & $\displaystyle\sum_t |g_t+\sigma_t|$ && MASX (MAS-Max)   & $\displaystyle\frac1N\sum_X \left|\frac{\partial (\max \textbf{q}_X)^2}{\partial \theta}\right| $
			%&$\surd$ 
			\\ 
			\bottomrule
		\end{tabular}
	\end{small}
	
	
	%\vskip -0.15in
\end{table}






\subsection{Memory Aware Synapses (MAS) and `Absolute Fisher Information'}\label{sec:memory}
We start by taking a closer look at the definition of the importances of MAS. We apply linearity of derivatives, the chain rule and write $y_0 = \argmax \mathbf{q}_X$ to obtain
\begin{eqnarray}\label{MAS1}
\frac{\partial \|  \textbf{q}_X \|^2}{\partial\theta} 
= 2\sum_{y\in Y} \textbf{q}_X(y) \frac{\partial \textbf{q}_X(y)}{\partial \theta}  
\approx 2 \textbf{q}_X(y_0)\frac{\partial \textbf{q}_X(y_0)}{\partial \theta} = 2 \textbf{q}^2_X(y_0)\frac{\partial \log \textbf{q}_X(y_0)}{\partial \theta}. %= 2 \textbf{q}^2_X(y_0) g(X,y_0)
\end{eqnarray}
Here we made the assumption that the sum is dominated by its maximum-likelihood label $y_0$, which should be the case if the network classifies its images confidently, i.e.\ $\textbf{q}(y_0)\gg \textbf{q}(y)$ for $y\neq y_0$. Recall that the importance is measured at the end of training, so that our assumption is justified  if the task has successfully been learned.
Using the same heuristic for the Fisher Information we obtain $$
\EE_{y\sim \textbf{q}_X}\left[g(X,y)^2\right] \approx \textbf{q}_X(	y_0) g(X,y_0)^2 = \textbf{q}_X(y_0) \left(\frac{\partial\log \textbf{q}_X(y_0)}{\partial\theta}\right)^2.
$$
Comparing this with \eqref{MAS1} makes the similarity between MAS and the Fisher Information apparent.
The only difference is that MAS has an additional factor of $2\textbf{q}_X(y_0)$ and that $g(X,y_0)$ is not squared.  
We therefore hypothesise that MAS is almost linearly dependent of the Absolute Fisher (AF), which is analogous to the Fisher Information, but takes absolute values of gradients rather than their squares, c.f.\ Table \ref{table:overview}. 

Our hypothesis is based on two assumptions: (a) The sum over the labels is dominated by its maximum likelihood label $y_0$, cf. equation \eqref{MAS1}. 
(b) We assume that the factor $2\textbf{q}_X(y_0)$ is roughly constant across most images $X$.

To check (a), we explicitly evaluate the term of the sum based on $y_0$ (and call this $\omega(\MASX)$, see Table \ref{table:overview}), and compare it to the entire sum (MASX vs MAS). See Figures \ref{figure:SI_scatter}A (top) and \ref{figure:correlations} (top) for strong empirical confirmations that the two measures are almost identical. 

 (b) is justified because at the end of training most images $X$ will have ${q}_X(y_0)\approx 1$. Note that even images with ${q}_X(y_0)=0.5$ deviate only by a factor of 2, and still lead to a large correlation between MAS and AF. As an empirical validation we check whether MASX and AF are linearly dependent.
Again, empirical evidence strongly supports this claim, see Figures \ref{figure:SI_scatter}A (middle\&bottom) and \ref{figure:correlations} (top). 






\subsection{Synaptic Intelligence (SI)}\label{sec:synaptic}
\subsubsection{Bias of Synaptic Intelligence}\label{bias}
To calculate $\omega(\SI)$, we need to calculate the product $p = \frac{\partial L(t)}{\partial \theta}\cdot\Delta(t)$ at each step $t$. Since evaluating the full gradient $\frac{\partial L(t)}{\partial \theta}$ is prohibitively expensive, SI \citep{zenke2017} uses a mini-batch. The resulting estimate is biased since the same mini-batch is used for the parameter update $\Delta(t)$ and the estimate of $\frac{\partial L(t)}{\partial \theta}$. 

We now give the calculations detailing the argument above.
For ease of exposition, let us assume that the network is optimized using vanilla SGD with learning rate $1$. 
%Very similar arguments apply to other optimizers. 
Given a mini-batch, denote its gradient estimate by $g+\sigma$, where $g=\frac{\partial L(t)}{\partial \theta}$ denotes the real gradient and $\sigma$ the mini-batch noise. With SGD the parameter update equals $\Delta(t) =  g+\sigma$. Thus, our product $p$ should be  
$p = g \cdot(g+\sigma).$ 
However, using $g+\sigma$, which was used for the parameter update, to estimate $\frac{\partial L(t)}{\partial \theta_i}$ results in 
$p_{biased} = (g+\sigma)^2.$ 
Thus, the gradient noise introduces a bias of
$\mathbb{E}[\sigma^2 +\sigma g] = \EE[\sigma^2].$

\paragraph{Unbiased Synaptic Intelligence.}
It is easy to design an unbiased estimate of $p$ by using two independent mini-batches to calculate the parameter update and to estimate $g$. This way we get $\Delta(t) =  g+\sigma$ and an estimate $g+\sigma'$ for $g$ from an independent mini-batch with independent noise $\sigma'$. We obtain
$
p_{unbiased} = (g+\sigma') \cdot (g+\sigma) 
$
which in expectation is equal to $p = g \cdot(g+\sigma).$
Based on this we define an unbiased importance measure
$$
\tilde{\omega_i}(\SIU) =  \sum_{t=0}^{T-1} (g_t+\sigma_t') \cdot \Delta(t). 
$$
%where the dash indicated that the gradient estimate is independent of the parameter update.

\paragraph{Bias-Only version of SI.}\label{bias_only}
To isolate the bias, we can simply take the difference between biased and unbiased estimate. Concretely, this gives a measure which only measures the bias of SI and is independent of the path integral, 
$$
\tilde{\omega_i}(\SIB) =   \sum_{t=0}^{T-1} ((g+\sigma)-(g+\sigma_t')) \cdot \Delta(t). 
$$ Observe that this estimate multiplies the parameter-update $\Delta(t)$ with nothing but stochastic gradient noise. From the perspective of SI, this should not be meaningful and have poor continual learning performance.


\paragraph{Which part dominates SI?}\label{exp:SI}
The approximations presented in equation (\ref{def_contribution}) imply that $L(0)-L(T)\approx\sum_i \tilde{\omega}_i(SI)$. Thus, comparing $\sum_i \tilde{\omega}_i$ for SI, SIU, SIB to $L(0)-L(T)$ measures how good the approximations are and shows whether SI is dominated by its bias, see Figure \ref{figure:summed_MNIST}. Further, comparing the continual learning performance of SI, SIU, SIB shows whether SI relies on the approximation of the path integral or its bias, see Table \ref{table:results}, Exp No 2.


\subsubsection{Synaptic Intelligence and Absolute Fisher Information}\label{sec:SI_FI}
In this section we will indicate the relation between the importance measure $\omega(\SI)$ and the Fisher Information.
Recall that $\omega(SI)$ is a sum over terms $\frac{\partial{L(t)}}{\partial \theta} \cdot \Delta(t)$, where $\Delta(t) = \theta(t+1) - \theta(t)$ is the parameter update at time $t$. Recall as well that both terms in this product, $\frac{\partial{L(t)}}{\partial \theta}$ as well as $\Delta(t)$, are computed/approximated using the same mini-batch and thus the have the same noise. 


For a precise understanding, we need to take into account how the optimizer uses stochastic gradients to update the parameters. The SI experiments (and ours) use the Adam optimizer \citep{kingma2014adam}. Given a stochastic gradient $g_t+\sigma_t$, 
it keeps a running average of the gradient $m_t = (1-\beta_1)(g_t+\sigma_t) + \beta_1 m_{t-1}$ as well as a running average of the squared gradients  $v_t = (1-\beta_2)(g_t+\sigma_t)^2 + \beta_2 v_{t-1}$. Ignoring some normalisation terms and the learning rate, the Adam parameter update is given by $\Delta(t) = m_t/(\sqrt{v_t} + \epsilon)$, where $\beta_1=0.9$ and $\beta_2 = 0.999$. Thus, 
\begin{eqnarray*}
	\frac{\partial L(t)}{\partial \theta} \Delta(t) = 
	%(g+\sigma)\cdot \frac{(1-\beta_1)(g+\sigma) + \beta_1 m_{t-1}}{\sqrt{v_t} + \epsilon} \\
	\frac{(1-\beta_1)(g_t+\sigma_t)^2}{{\sqrt{v_t} + \epsilon}} + \frac{\beta_1(g_t+\sigma_t)m_{t-1}}{{\sqrt{v_t} + \epsilon}}.
\end{eqnarray*}
Assuming that the noise $\sigma_t$ is considerably bigger than the gradient $g_t$  we obtain
\begin{eqnarray}\label{eq:noise}
\frac{\partial L(t)}{\partial \theta}\Delta(t) 
%=  (1-\beta_1) \frac{(g_t+\sigma_t)^2}{{\sqrt{v_t} + \epsilon}} + \beta_1\frac{g_t()}{{\sqrt{v_t} + \epsilon}}   
\approx (1-\beta_1)\frac{(g_t+\sigma_t)^2}{{\sqrt{v_t} + \epsilon}} \label{eq:main_SI_bias} %\nonumber
\end{eqnarray}
The assumption made here is $(1-\beta_1)\sigma_t^2\gg \beta_1 m_{t-1}g_t$ (we ignore the term $\sigma_t m_{t-1}$ since $\EE[\sigma_t m_{t-1}]=0$ and since we average SI over many time steps). This assumption is supported strongly by Figure \ref{figure:summed_MNIST}, where the difference between green (SI) and blue (SIU) line is caused precisely by $(1-\beta_1)\sigma^2$, see \ref{sec:calc_bias} for full details. We also refer to \citep{lan2019} and Figures \ref{figure:noise}, \ref{figure:noise_cdf} and \ref{figure:summed_cifar_all}, \ref{figure:summed_mnist_all}  for more evidence that the noise is considerably bigger than the gradient.

%are summed over time. 
%In addition, the denominator $\sqrt{v_t}$ changes only slowly (since $\beta_2=0.999$) 
%and is roughly equal to $\sqrt{\EE[(g_t+\sigma_t)^2]}$ across time. Therefore, 

Next, we consider $v_t$. It is a slowly moving exponential average of $(g_t+\sigma_t)^2$ and will therefore be approximately $\EE[(g_t+\sigma_t)^2]$. It is thus reasonable to expect that $\sqrt{v_t}$ is roughly proportional to $|g_t+\sigma_t|$. This clearly does not hold for all possible distributions of $g_t+\sigma_t$, but is unlikely to be violated by non adversarially chosen, realistic distributions. 
With \eqref{eq:noise} and $\sqrt{v_t}\appropto |g_t+\sigma_t|$ we arrive at 
\begin{eqnarray}\label{eq:SI-OnAF}
	\tilde{\omega}(SI) =\sum_t \frac{\partial L(t)}{\partial \theta}\Delta(t)\approx (1-\beta_1)\sum_t \frac{(g_t+\sigma_t)^2 }{\sqrt{v_t}} 
	%\propto \frac{\EE[(g_t+\sigma_t)^2]}{\sqrt{\EE[(g_t+\sigma_t)^2]}}
	\appropto \sum_t |g_t+\sigma_t|.
\end{eqnarray}

\iffalse
In SI, %the products 
$\frac{\partial{L(t)}}{\partial \theta} \cdot \Delta(t)$ is summed over time.
Moreover, $v_t$ is roughly  equal to $\EE[(g_t+\sigma_t)^2]$. Thus,
\begin{eqnarray*}
	\tilde{\omega}(SI) \approx (1-\beta_1)\sum_t \frac{(g_t+\sigma_t)^2 }{\sqrt{\EE[(g_t+\sigma_t)^2]}} 
	%\propto \frac{\EE[(g_t+\sigma_t)^2]}{\sqrt{\EE[(g_t+\sigma_t)^2]}}
	\appropto \sum_t |g_t+\sigma_t|.
\end{eqnarray*}
The last approximation assumes that $\sqrt{\EE[(g_t+\sigma_t)^2]}$ is approximately proportional to the magnitude $|g_t+\sigma_t|$ of a typical gradient, which seems rather plausible in a non-adversarial setting but is of course not true for all distributions of $g_t+\sigma_t$.
\fi
An alternative way to arrive at \eqref{eq:SI-OnAF} is following the analysis of \cite{balles2018dissecting}, who show that the update of Adam is mostly given by the sign of the moment $m_t$.
Our resulting approximation $\tilde{\omega}(SI)\appropto \sum_t |g_t+\sigma_t|$ is very similar to the (Empirical) Absolute Fisher. The only differences are (a) the gradient in $\tilde{\omega}(SI)$ is evaluated in mini-batches rather than on single images; (b) the sum is taken `online' along the parameter trajectory rather than at the final point of the trajectory. (a) does not have a large effect %(other than rescaling by the batch size)
when $\sigma_t\gg g_t$ (as detailed in \ref{sec:calc_batch}) which we have seen to be the case.
The influence of (b) is hard to quantify and depends on how much the gradients change along the parameter trajectory.
To capture this difference, we define the Online Absolute Fisher as 
$
\tilde{\omega} (\OnAF) = \sum_t |g+\sigma_t|
$
and empirically test how similar %$\tilde{\omega}(SI), \tilde{\omega}(\OnAF)$ as well as 
$\tilde{\omega}(\OnAF)$ and $\tilde{\omega}(\AF)$ are. The fact that Adam usually works well with $\beta_2=0.999$ suggests that the second moment of the gradient and thus OnAF change very slowly in many settings, indicating that OnAF and AF are often and robustly similar.

Our heuristics suggest that $\tilde{\omega}(\SI)$ and $\tilde{\omega}(\OnAF)$ are very similar. If in addition, we empirically see that $\tilde{\omega}(\OnAF)$ and $\tilde{\omega}(\AF)$ are similar, then SI approximates AF, a rescaling of the Fisher.  Figures \ref{figure:SI_scatter}B and \ref{figure:correlations}  empirically confirm both parts of this hypothesis. 


We emphasise that our derivation above assumes that the parameter update $\Delta(t)$ is given by the gradients of the current task and ignores influence of regularisation on parameter updates. The latter will change update direction and momentum of the optimizer. Thus, strong regularisation will make the relation between SI and OnAF noisy, but not abolish it. 
See Fig \ref{figure:correlations} (middle row) and Appendix \ref{sec:effect_reg_SI} for various confirmations hereof.% for controls. %experiments.%showing that SI, SIB are more related to AF than SIU (and more effective at continual learning).




\begin{figure}[t]
	\begin{center}
		\begin{subfigure}{0.52\textwidth}
			%\vskip 0.1in
			\centerline{\includegraphics[width=\textwidth]{../figures/summed_contributions_mnist.png}}
			\vskip -0.05in
			\caption{}
			\label{figure:summed_MNIST}
		\end{subfigure}
		\begin{subfigure}{0.45\textwidth}
			\centerline{\includegraphics[width=\textwidth]{../figures/correlations_MAS.png}}
			\vskip -0.05in
			\centerline{\includegraphics[width=\textwidth]{../figures/correlations_SI_MAS.png}}
			\vskip -0.05in
			\caption{}
			\label{figure:correlations}
		\end{subfigure}
		\vskip -0.1in
		\caption{
			\textbf{(a)} \textbf{Summed importances} $\sum_i \tilde{\omega}_i$ for Permuted-MNIST.  
			\textbf{(b)} \textbf{Pearson correlations of importances for all tasks.} Dashed lines represent CIFAR, solid lines MNIST. Error bars are stds for 4 runs. `AF' is an estimates the Absolute Fisher with 30000 (MNIST) resp.\ 5000 (CIFAR) images. `AF\_small', `MAS' and `MASX' use 1000 resp.\ 500 images.
		}
	\end{center}
	\vskip -0.2in
\end{figure}



==> ic/sections/05_experiments.tex <==
\section{Experiments}\label{sec:experiments}
In this section we empirically test our three main hypotheses:
\begin{enumerate}
	\item Does Memory Aware Synapses approximate the Absolute Fisher as derived in Sec \ref{sec:memory}?
	\item Which part of the importance $\tilde{\omega}(SI)$ of Synaptic Intelligence, the bias or the unbiased contribution, explains its effectiveness, see Section \ref{bias}?
	\item Does $\tilde{\omega}(SI)$ correlate strongly with  the Absolute Fisher as indicated in Sec \ref{sec:SI_FI}?
\end{enumerate}
%Our affirmative answers to question 1.\ and 3.\ suggest that both Memory Aware Synapses (MAS) and Synaptic Intelligence (SI) work because they approximate a rescaled version of the Fisher Information, which is a somewhat sound theoretical explanation for their effectiveness. At the same time, it raises the question whether the rescaled version (i.e.\ Absolute Fisher) or the original Fisher Information is more effective, which is the last question we investigate.  



\subsection{Experimental Setup}
Our experiments closely follow \citep{zenke2017}. We use the \textbf{Permuted MNIST} \citep{goodfellow2013} benchmark with 10 tasks, a fully connected ReLU architecture and a single output-head (`domain incremental' setting, c.f.\ \citep{hsu2018,van2019}) and the \textbf{Split CIFAR 10/100} benchmark with the keras default CNN and a multi-head output (`task incremental').  
Following \citep{swaroop2019}, but unlike \citep{zenke2017}, we re-initialise model variables (fully connected layers, etc.) after each task and usually find better performance in our hyperparameter searchers.
We defer further experimental details to the Appendix \ref{sec:exp_detail}. Code is available on github\footnote{\url{https://github.com/freedbee/continual_regularisation}}.

%How similar AF and OnAF are depends on how quickly the gradient changes along the parameter trajectory. 
\begin{figure}[t]
	\vskip -8pt
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/MAS_MASX_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure}
	\hspace{6pt}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_OnAF_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/OnAF_AF_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_AF_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure} 
	
	\vskip -0.2in
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/MAS_AF_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure}
	\hspace{6pt}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_OnAF_int_CIFAR_task_6.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/OnAF_AF_int_CIFAR_task_6.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_AF_int_CIFAR_task_6.png}}
		\end{center}
	\end{subfigure} 
	\vskip -0.2in
	
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/MAS_AF_int_MNIST_task_5.png}}
		\end{center}
	\end{subfigure}
	\hspace{6pt}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_OnAF_int_MNIST_task_5.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/OnAF_AF_big_int_MNIST_task_5.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_AF_big_int_MNIST_task_5.png}}
		\end{center}
	\end{subfigure} 
	\vskip -0.3in
	\caption{
		\textbf{Scatter- and Intensity plots for pairs of importance measures.} 
		$r$ denotes the Pearson correlation.
		\textit{Scatter Plots (blue):} Each point in the scatter plot corresponds to one weight of the net. A straight line through the origin corresponds to two importances measures being multiples of each other. 
		\textit{Intensity Plots (gray scale):} Show data analogous to scatter plots, but are normalised for better visualisation. See \ref{sec:intensity} for details and Fig \ref{fig:scatter_app} for same data with only scatter/intensity plots.
		\textbf{(A)} Comparison between MAS, MASX, AF. 
		\textbf{(B)} Comparison between SI, OnAF, AF on first task of CIFAR (top),  last task of CIFAR (middle) and `middle' task of MNIST (bottom). See Fig \ref{figure:correlations} for data on all tasks.}
	\label{figure:SI_scatter}
	\vskip -0.1in
\end{figure}

%and we will assess empirically how strong the correlation between OnAF and AF as well as whether our heuristics 

%We note that our derivation for the similarity of SI and OnAF relies on the approximation made in \eqref{eq:main_SI_bias}, which is due to the bias of SI.

%We empirically assess the correlation between $\tilde{\omega}(SI)$ and $\tilde{\omega}(\OnAF)$ as well as the difference between SI and Absolute Fisher in Figure \ref{figure:SI_scatter}.





\subsection{Results}
\paragraph{MAS and Absolute Fisher.}
Our first objective is to test whether MAS and Absolute Fisher are related. To this end we  calculate $\omega(\MAS)$, $\omega(\MASX)$, $\omega(\AF)$  and show scatter plots of these values in Figure \ref{figure:SI_scatter} \textbf{(A)}. We  find that they are almost identical. Figure \ref{figure:correlations} shows equally strong correlations on the other tasks and datasets, presenting strong evidence for our heuristics.
We also evaluated continual learning algorithms based on $\omega(\MAS)$, $\omega(\MASX),$ $\omega(\AF)$ and found very similar results, Table see \ref{table:results}, Exp No 1, providing further evidence that our mathematical derivations hold.

\paragraph{Why does SI work?}
To understand how large the bias of SI is, we track the sum $\sum_{i} \tilde{\omega}_i$ of importances for SI and its unbiased version SIU. As a control we 
include the decrease of the loss $L(0)-L(T)$ which the path-integral (c.f.\ equation (\ref{def_contribution})) approximates, as well as an first order approximation of the path-integral without relying on stochastic gradient estimates (computing the full training set gradient at each step). The results are portrayed in Figure \ref{figure:summed_MNIST}. They indicate that (1) the bias is 5-6 times larger than the unbiased part;  (2) using an unbiased gradient estimate and using the entire training set gradient gives almost identical values of $\sum_i\omega_i$ supporting the validity of the unbiased estimator; (3) even the unbiased first order approximation of the path integral overestimates the decrease in loss. This is consistent with previous empirical studies showing that the loss has positive curvature \citep{jastrzebski2018relation, lan2019}.  See Figures \ref{figure:summed_cifar_all}, \ref{figure:summed_mnist_all} for similar results on CIFAR and other MNIST tasks.

We have seen that the SI's bias is considerably larger than its unbiased component. This does not fully explain which of these parts is more essential for continual learning. We therefore run continual learning algorithms based on SI, its unbiased version (SIU) as well as a version which isolates the bias (SIB). The results are shown in Table \ref{table:results}, Exp No.\ 2. SIU consistently has worse performance than SI and SIB has the same or slightly better performance than SI. From SI's perspective this is rather surprising and is convincing evidence that SI's continual learning capability is due to its bias.






\paragraph{Is SI related to Absolute Fisher?} Our main assumption in relating SI to Online Absolute Fisher (OnAF) was that the contribution of the  noise (bias) to SI is bigger than its unbiased part, c.f.\ equation \eqref{eq:noise}. We have already seen strong evidence that this is the case (Figure \ref{figure:summed_MNIST}). Therefore it may be expected that OnAF and SI do have significant correlations: On all tasks of MNIST and the first task of CIFAR, SI and OnAF have (Pearson) correlations $>0.93$; on tasks 2-6 of CIFAR we find weaker, but significant correlations around 0.5, see Figures \ref{figure:SI_scatter}, \ref{figure:correlations}. This weaker correlation on CIFAR tasks 2-6 is well explained by regularisation, see \ref{sec:SI_FI} and Appendix \ref{sec:effect_reg_SI} for two control experiments. 

We also find that OnAF and AF are surprisingly similar, thus closely relating SI and AF (Figures \ref{figure:SI_scatter}, \ref{figure:correlations}) supporting our hypotheses.\footnote{ We check in \ref{sec:training_time} that similarity of AF, OnAF does not depend on how long the networks are trained and show control correlations between SIU, SIB and (On)AF in \ref{sec:controls}, further supporting our claim, that continual learning performance is explained by similarity to AF.}
We also evaluate the corresponding continual learning algorithms SI, OnAF and AF, see Table \ref{table:results}, Exp 3. The results are very similar, indicating that SI, like MAS, works because it approximates a rescaled version of the Fisher Information. %We believe that the slight gap between performance of SI, OnAF as compared to AF on CIFAR is due to the normalisation of SI and OnAF given in equation (\ref{eq:rescale}), see appendix for an ablation experiment.





\paragraph{Is Absolute or Real Fisher better for continual learning?}
We have seen evidence that both MAS and SI rely on estimating a rescaled Fisher Information. This raises the questions whether a rescaled version of the Fisher or the Fisher itself are more effective for continual learning. To answer this, we compare MAS, AF  and EWC, since these methods all evaluate the importance at the end of training. 
The results are shown in Figure \ref{table:results}, Exp 4. All algorithms perform similarly, only the difference between MAS and EWC on CIFAR is significant ($p=0.04$, t-test, not corrected for multiple comparisons). Which algorithm performs best may well depend on hyperparameters and the precise training set-up.

%We find, maybe surprisingly, that on both continual learning tasks P-MNIST, and CIFAR 10/100 the rescaled, Absolute Fisher has slightly better performance. However, we can not exclude the possibility that this observation is data-set dependent.










\begin{table}[t]
	%\vskip -12pt
	\caption{\textbf{Test accuracies on Permuted-MNIST and Split CIFAR 10/100.} 
		Algorithms are grouped by experiment as indicated in main text.
		Reported results are mean and standard deviation over 3 resp. 10 runs for P-MNIST resp.\ CIFAR 10/100. 
	}
	\label{table:results}
	\vskip -0.2in
	\begin{center}
		%\vskip -0.2in
		\begin{small}
			%\vskip -0.1in
			\begin{sc}
				%\vskip -0.1in
				\begin{tabular}{cccc|c|cccc}
					\toprule
					\textbf{No.} & \textbf{Algo.} & \textbf{P-MNIST} & \textbf{CIFAR} & &\textbf{No.} & \textbf{Algo.} & \textbf{P-MNIST} & \textbf{CIFAR} \\
					\midrule
					\multirow{3}*{1}
					&  $\MAS$ & 97.3 $\pm$ 0.1& 73.7 $\pm$ 0.5 & &\multirow{3}*{3} & $\SI$ & 97.2 $\pm$ 0.1& 74.4 $\pm$ 0.5\\
					& $\MASX$ & 97.4 $\pm$ 0.2& 73.7 $\pm$ 0.2 &
					&& $\OnAF$& 97.3 $\pm$ 0.1&    74.4 $\pm$ 0.6 \\ 
					& $\AF$ & 97.4 $\pm$ 0.1& 73.4 $\pm$ 0.4&
					&& $\AF$ & 97.4 $\pm$ 0.1& 73.4 $\pm$ 0.4\\ 
					\midrule
					\multirow{3}*{2}
					& $\SI$ & 97.2 $\pm$ 0.1& 74.4 $\pm$ 0.5& 
					&\multirow{3}*{4} 
					& $\EWC$ & 97.2 $\pm$ 0.2& 73.1 $\pm$ 0.7 \\
					& $\SIU$ & 96.3 $\pm$ 0.1& 72.5 $\pm$ 0.8& 
					&&   $\MAS$ & 97.3 $\pm$ 0.1& 73.7 $\pm$ 0.5    \\
					& $\SIB$ & 97.2 $\pm$ 0.1& 75.1 $\pm$ 0.4&
					&& $\AF$ & 97.4 $\pm$ 0.1& 73.4 $\pm$ 0.4 \\
					\bottomrule
				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
	\vskip -0.3in
\end{table}









==> ic/sections/C_AF_F.tex <==
\section{Relation between Absolute Fisher and Real Fisher}
It remains to investigate the relation of Absolute and Real Fisher. Recall that (taking expectations over inputs and predicted labels) the diagonal Fisher is defined as $\F = \EE[|g+\sigma|^2]$ while the diagonal Absolute Fisher is defined as $\AF = \EE[|g+\sigma|]$, where $g+\sigma$ is the (stochastic) gradient. 

Empirically, we see that $\AF$ and $\F$ are highly correlated, see Figure \ref{figure:AF_F} left. 

Theoretically, the exact relationship of Fisher and Absolute Fisher depends on the gradient distribution. If, for example, gradients are distributed normally $(g+\sigma)\sim\mathcal{N}(\mu, \Sigma)$ with $\Sigma_{i,i} \gg \mu_i$ (corresponding to the observation that the noise is much bigger than the gradients), we obtain $\F_i \approx \Sigma_{i,i}$ and (since $|g+\sigma|$ follows a folded normal distribution) we also have $\AF_i \approx c \sqrt{\Sigma_{ii}}$ with $c=\sqrt{2/\pi}$. Thus, in the case of a normal distribution with large noise, we have $\F \appropto (\AF)^2$. The relationship $\F \propto (\AF)^2$ is in fact what we empirically observe on Split CIFAR, where correlations between $(\AF)^2$ and $\F$ are $>0.98$ for all tasks and repetitions, and partly on P-MNIST, where correlations between $(\AF)^2$ and $\F$ are between 0.86 and 0.96. 
 
 
  \begin{figure}[h]
 	%\vskip -40pt
 	\begin{center}
 		\begin{subfigure}{0.23\textwidth}
 			%\vskip 1in
 			\centerline{\includegraphics[width=\textwidth]{../figures/correlations_CIFAR_AF_F.png}}
 			\centerline{\includegraphics[width=\textwidth]{../figures/correlations_MNIST_AF_F.png}}
 		\end{subfigure}
 		\begin{subfigure}{0.23\textwidth}
 			\centerline{\includegraphics[width=\textwidth]{../figures/AF_F_scatter_CIFAR_task_1.png}}
 		\end{subfigure}
 	\begin{subfigure}{0.23\textwidth}
 		\centerline{\includegraphics[width=\textwidth]{../figures/AF_F_scatter_MNIST_task_1.png}}
 	\end{subfigure}
	 \begin{subfigure}{0.23\textwidth}
	 	\centerline{\includegraphics[width=\textwidth]{../figures/AF_F_scatter_MNIST_task_10.png}}
	 \end{subfigure}
 	\end{center}
 	\vskip -16pt
 	\caption{
 		\textbf{Empirical Relation between Absolute Fisher and Real Fisher.} 
 		\textbf{Left}: Note y-axis range. Summary of Pearson Correlations (top: CIFAR, bottom: MNIST), error bars represent std over 4 runs. \textbf{Mid - Right}: Example scatter plots. Relation on Split CIFAR is nearly quadratic across tasks and repetitions. There is more variation on P-MNIST (two extremes shown). Yellow lines show least-squares fit of the model $f(x)=ax^2$ with parameter $a$.
 	}
 	\label{figure:AF_F}
 	%\vskip -0.2in
 \end{figure}
 
 
 
 
 
 
 
 
 
 
 
 

 
 
 
 
 
 
 


==> ic/sections/X_00_abstract.tex <==
\begin{abstract}%   <- trailing '%' for backward compatibility of .sty file
Continual Learning addresses the challenge of learning a number of different distributions sequentially. The goal of maintaining knowledge of earlier distributions without re-accessing them starkly conflicts with standard SGD training for artificial neural networks. 
%Continual Learning addresses the challenge of learning different distributions sequentially without revisiting data from old distributions but also without overwriting previous knowledge -- an objective in conflict with standard SGD training for artificial neural networks. 
An influential method to tackle this are so-called regularisation approaches. They measure the importance of each parameter for modelling a given distribution and subsequently protect important parameters from large changes. 
In the literature, three ways to measure parameter importance have been put forward and they have inspired a large body of follow-up work. % combining and extending their key ideas. 
Here, we present strong theoretical and empirical evidence that these three methods, Elastic Weight Consolidation (EWC), Synaptic Intelligence (SI) and Memory Aware Synapses (MAS), all approximate the Fisher Information. %to measure parameter importance. 
Only EWC intentionally relies on the Fisher, while the other two methods stem from rather different motivations. We find that for SI the relation to the Fisher -- and in fact its performance -- is due to a previously unnoticed bias.
Altogether, this unifies a large body of regularisation approaches. It also provides the first theoretical explanation the effectiveness of SI- and MAS-based algorithms and offers new, theoretically justified versions of these algorithms. 
From a practical viewpoint, our insights offer computational speed-ups and uncover conditions needed for different algorithms to work.

\end{abstract}

\iffalse
\begin{keywords}
  Continual Learning, Regularisation, Fisher Information
\end{keywords}
\fi


==> ic/sections/X_01_introduction.tex <==

\section{Introduction}
\label{introduction}

Despite considerable progress, many gaps between biological and machine intelligence remain. Animals, for example, flexibly learn new tasks throughout their lives, while at the same time maintaining robust memories of previous knowledge. This ability conflicts with traditional training procedures for artificial neural networks, which overwrite previous skills when optimizing new tasks \citep{mccloskey1989, goodfellow2013}. The field of continual learning is dedicated to mitigate this crucial shortcoming of machine learning. It exposes neural networks to a sequence of distinct tasks. During training new tasks, the algorithm is not allowed to revisit old data, but should retain previous skills while remaining flexible enough to also acquire new knowledge.

An influential line of work to approach this challenge was introduced by \cite{kirkpatrick2017}, who proposed the first regularisation-algorithm, Elastic Weight Consolidation (EWC). After training a task, EWC measures the importance of each parameter and introduces an auxiliary loss penalising large changes in important parameters. Naturally, this raises the question of how to measure this `importance'. While EWC uses the diagonal Fisher Information, two alternatives have been proposed: Synaptic Intelligence (SI, \citet{zenke2017}) aims to attribute the decrease in loss during training to individual parameters  and Memory Aware Synapses (MAS, \citet{aljundi2018}) introduces a heuristic measure of output sensitivity. Together, these three approaches have inspired many further regularisation-based approaches, including combinations of them \citep{chaudhry2018}, refinements \citep{huszar2018, ritter2018, chaudhry2018, yin2020sola}, extensions \citep{schwarz2018, liu2018rotate, park2019continual, lee2020continual} and applications in different continual learning settings \citep{aljundi2019task} as well as different domains of machine learning \citep{lan2019}. Almost every new continual learning method compares to at least one of EWC, SI and MAS. 

Despite their popularity and influence, basic practical and theoretical questions regarding these algorithms had previously been unanswered. Notably, it was unkown how similar these importance measures are. Additionally, for SI and MAS (and their follow-ups) there was no solid theoretical understanding of their effectiveness. 
Here, we close both these gaps and show that SI and MAS, despite seemingly orthogonal motivations, approximate a version of the Fisher Information.  
Our methods combine theoretical analyses with fine-grained empirical validations on standard continual learning benchmarks.
This also leads to several new regularisation approaches, offering computational speed-ups or theoretically sound alternatives to existing algorithms.
In the case of SI, we identify a previously unnoticed bias in its approximation. We then show that this bias is responsible for the algorithms performance and for its tie to the Fisher Information. One of the algorithms developed to establish this result additionally  offers applications outside continual learning \citep{lan2019}.

%and demonstrate that the tie to the Fisher is due to a biased approximation of its original objective. Removing the bias hurts performance, while removing the original objective (keeping only the bias) restores or slightly improves performance. 

%To establish our claims, we show theoretically how SI and MAS are related to the Fisher Information and then empirically confirm that each of our approximations is justified on standard continual learning benchmarks. 

Our results unify the regularisation approaches proposed so far; they theoretically explain why SI- and MAS-based algorithms are effective and introduce justified, more efficient alternatives to existing algorithms; our insights also help to predict under which circumstances algorithms will perform well.

\iffalse
- emphasise CL importance in beginning\\
- too much detail on algorithms?\\
- introduce new, more interpretable/justified algorithms\\
- theory \\
- explicitly name experiments: Bias experiment, CL performance experiments, correlation experiments \\
organisation: review of existing + MAS (theory + exp) + SI(theory + exp) + new algorithms(batch-fisher, OnAF, SIU)
\fi






\iffalse
Despite much progress, there remain many gaps between artificial and biological intelligence. Among these, the ability of animals to acquire new skills throughout their life takes, while also storing robust memories
 a prominent role and starkly contrasts with `catastrophic forgetting' observed in neural networks
%while maintaining robust memories of past abilities
 %has inspired a growing body of work in the machine learning literature. 
The field of continual learning (CL) is dedicated to solve this shortcoming and has gained increased interest in recent years. 

In CL, a number of tasks are presented sequentially and the algorithm should learn new tasks without overwriting previous knowledge and without revisiting old data. 
This is challenging since standard SGD based optimization simply overwrites the networks previous knowledge when training on new tasks \citep{mccloskey1989, goodfellow2013}. 

An important class of algorithms proposed to solve this problem are regularisation approaches \citep{kirkpatrick2017, zenke2017, aljundi2018, ritter2018, chaudhry2018, huszar2018, schwarz2018, nguyen2017}. They identify important weights after each task and protect them from large changes by modifying the loss function.
At the heart of these algorithms lies the question how to estimate parameter importance, as this directly determines which parameters will be kept close to their old value and which parameters can be modified freely to solve new tasks. 




In this article, our aim is to understand why different importance measures proposed in the literature are effective. Notably, this question had remained open for two well-known regularisation methods, Synaptic Intelligence (SI) \citep{zenke2017} and Memory Aware Synapses (MAS) \citep{aljundi2018}. The latter approach has a purely heuristic motivation, while the former makes simplifying assumptions, violated in a deep learning setting, to theoretically justify its importance measure.


Our main contribution is to provide mathematical as well as empirical evidence that both these methods, SI and MAS, despite their different motivations, approximate a rescaled version of the Fisher Information. The Fisher Information has been used for continual learning \citep{kirkpatrick2017} along with a clear theoretical, Bayesian justification \citep{kirkpatrick2017, huszar2018}.  
Thus, on top of unifying different regularisation-approaches proposed so far, our results give a more sound theoretical explanation for the effectiveness of two more continual learning algorithms.

To establish our claims, we  first investigate MAS and give a simple mathematical derivation to show that MAS approximates what we call the Absolute Fisher. We carefully validate  the assumptions of our derivations as well as the resulting claims empirically on standard continual learning benchmarks.
As a second -- maybe surprising -- step we show that the importance approximation of SI  is biased and that this bias contributes most to the continual learning performance of SI. Finally, we show that through this bias SI is -- like MAS -- closely related to the Absolute Fisher.  


%In addition, we point out that one of our algorithms `Unbiased Synaptic Intelligence' (SIU) also has an application outside continual learning. 
%Namely, SIU is an unbiased approximation of the recently proposed Loss-Change-Allocation (LCA) method \citep{lan2019}, which assesses how much individual parameters contribute to performance improvement during training. The authors show that LCA gives interesting empirical insights in the complex learning process of neural networks. However, in its original version, the method requires calculating the gradient on the entire training set at least once per parameter update. In contrast, our approximation only requires evaluating the gradient on a mini-batch, which allows using Loss-Change-Allocation for larger, more complex datasets.
\fi

==> ic/sections/X_02_related_work.tex <==
\section{Related Work}
The problem of catastrophic forgetting in neural networks has been studied for many decades \citep{mccloskey1989, ratcliff1990, french1999}.
In the context of deep learning, it received more attention again
\citep{goodfellow2013, srivastava2013}.
All previous work we are aware of proposes new or modified algorithms to tackle continual learning. No attention has been directed towards understanding or unifying existing methods and we hope that our work will not remain the only effort of this kind. %With the myriad of existing algorithms, we believe this to be a worthwhile goal. Below we survey some of the existing algorithms.
%
We now review the broad body of continual learning algorithms.
Following \citep{parisi2019}, they are  often categorised into regularisation-, replay- and architectural approaches. 
%
Most \textit{regularisation methods} will be reviewed more closely in the next section. There we cover regularisation for standard neural nets, but the same idea has also been applied to bayesian neural networks \citep{nguyen2017, swaroop2019}. An alternative approach \citep{mirzadeh2020understanding} does not penalize deviating from important parameters, but rather modifies training so that the network is robust to such deviations.
%
\textit{Replay methods} refer to algorithms which either store a small sample or generate data of old distributions and use this data while training on new methods \citep{rebuffi2017, lopez2017, shin2017, kemker2017}. These approaches can be seen as investigating how far standard i.i.d.-training can be relaxed towards the (highly non-i.i.d.)\ continual learning setting without losing too much performance. They are interesting, but usually circumvent the original motivation of continual learning to maintain knowledge \textit{without} accessing old distributions. Intriguingly, the most effective way to use old data appears to be simply replaying it, i.e.\ mimicking training with i.i.d.\ batches sampled from all tasks simultaneously \citep{chaudhry2019continual}.
%
\textit{Architectural methods} extend the network as new tasks arrive \citep{fernando2017, li2019, schwarz2018, golkar2019continual, von2019continual}. This can be seen as a study of how old parts of the network can be effectively used to solve new tasks and touches upon transfer learning. Typically, it avoids the challenge of integrating new knowledge into an existing networks.
%
Finally, \cite{van2019, hsu2018, farquhar2018} point out that  different continual learning scenarios and assumptions with varying difficulty were used across the literature.%They also clearly define and distinguish these scenarios and test how well different algorithms perform in them.
\footnote{In the appendix, we critically review and question some of their experimental results.}


\iffalse
%An attempt to overcome this problem was made with the algorithm Elastic Weight Consolidation (EWC) \citep{kirkpatrick2017}. 
%We will review EWC and two other regularisation approaches -- Synaptic Intelligence \citep{zenke2017} and Memory Aware Synapses \citep{aljundi2018} -- as well as their relatives \citep{ritter2018, chaudhry2018, schwarz2018} more closely in the next section. 
%The idea of regularisation was also applied in the context of Bayesian neural networks in \citep{nguyen2017,swaroop2019}, who
%use the weights' posteriors after having learned a task as the prior for learning the next task.  

On top of regularisation approaches,  \citet{parisi2019} identify two more classes of continual learning approaches.

One of these classes are replay methods, which rely on data from old distributions to protect knowledge while learning new tasks.
For example, iCarl \citep{rebuffi2017} uses stored datapoints from old datasets and computes nearest neighbours in feature space for classification. GEM \citep{lopez2017} and follow up work \citep{chaudhry2018efficient, aljundi2019}  project gradients from new tasks onto directions that do not increase the loss on stored examples. However, empirical results from \citep{chaudhry2019continual} suggest that one of the most effective ways to use small samples of old data is to simply mix them with the mini-batches of new data during training.
To avoid storing old examples, which strictly speaking violates continual learning desiderata, \textit{generative replay} methods train generative models to simulate old data distributions \citep{shin2017}. In this context, biologically inspired replay systems which mimic the hippocampus have also been put forward \citep{kemker2017}.

The third class of continual learning algorithms are  architectural approaches, which use network expansion to learn new tasks without corrupting previous knowledge. PathNet \citep{fernando2017} uses evolution to identify good subnetworks for each individual tasks, while \citep{li2019} extends the network through neural architecture search. \citep{schwarz2018, golkar2019continual} first train on a task, then compress the resulting net and iterate this process. Mixture models, with growing numbers of components, are investigated in \citep{rao2019, lee2020}.







Before reviewing the continual learning literature
we point out that one of our algorithms is linked to the recently proposed Loss-Change-Allocation (LCA) \citep{lan2019}. This method gains insights into the training process of neural networks \citep{alain2016, raghu2017, shwartz2017} by assessing how much the changes of individual parameters contribute to learning. To this end, LCA approximates the same path integral as Synaptic Intelligence \citep{zenke2017}. For the approximation, the gradient has to be evaluated on the entire training set  for each parameter update. Our method `Unbiased Synaptic Intelligence' gives an unbiased estimate of the same quantity, but only using mini-batches, thus being computationally cheaper.



%As pointed out, one of our algorithms, `Unbiased Synaptic Intelligence', is closely related to the recent Loss-Change-Allocation algorithm \citep{lan2019}. This work gives interesting insights into the training process of neural nets and as such joins empirical investigations like \citep{alain2016, raghu2017, shwartz2017}.

\fi

==> ic/sections/X_03_regularisation.tex <==
\section{Review of Existing Regularisation Methods}
\subsection{Formal Description of Continual Learning}
In continual learning we are given $K$ datasets $\mathcal{D}_1,\ldots,\mathcal{D}_K$ sequentially. When training a neural net with $N$ parameters $\theta\in \mathbb{R}^N$ on dataset $\mathcal{D}_k$, we have no access to the previously seen datasets $\mathcal{D}_{1:k-1}$. However, at test time the algorithms is tested on all $K$ tasks, usually the average accuracy is taken as measure of the algorithms performance, but see also \cite{chaudhry2018}.






\subsection{Common Framework for Regularisation Methods}
\iffalse
Regularisation based  approaches introduced in  \citep{kirkpatrick2017, huszar2018} protect previous memories by modifying the loss function $L_k$ related to dataset $\mathcal{D}_k$. Let us denote the parameters obtained after finishing training on task $k$ by $\theta^{(k)}$ and let  $\Omega^{(k)}$ be a positive semi-definite $N\times N$ matrix encoding parameter importance. When training on task $k$, regularisation methods use the loss 
\begin{eqnarray}\label{eq:regularisation}
\tilde{L}_k = L_k + c\cdot \left(\theta - \theta^{(k-1)}\right)^T \Omega^{(k-1)} \left(\theta-\theta^{(k-1)}\right).
\end{eqnarray}
where $c>0$ is a hyperparameter. The first term is the standard loss on task $k$. The second term makes sure that parameters do not move away too far from their previous values.

It can already be seen that the matrix $\Omega^{(k)}$ is prohibitively large for moderately sized networks, as it has $N^2$ entries, where $N$ is the number of parameters. $\Omega$ is therefore often approximated by its diagonal $diag(\omega_1,\ldots, \omega_N)$. The loss then simplifies to
\[
\tilde{L}_k = L_k + c\cdot \sum_{i=1}^N \omega_i ^{(k-1)}\left(\theta_i - \theta^{(k-1)}_i\right)^2
\]
and $\omega_i$ is often referred to as the importance of the $i$-th parameter $\theta_i$. 
Usually, we have $\omega_i^{(k)} = \omega_i^{(k-1)} + \omega_i$, where $\omega_i$ is the importance for the most recently learned task $k$.

How good a regularisation based approach is, depends on its importance estimates $\omega_i$. The contribution of this work is to understand why different measures work and how similar they are.

\fi
Regularisation based  approaches introduced in  \cite{kirkpatrick2017, huszar2018} protect previous memories by modifying the loss function $L_k$ related to dataset $\mathcal{D}_k$. Let us denote the parameters obtained after finishing training on task $k$ by $\theta^{(k)}$ and let  $\omega^{(k)}\in \mathbb{R}^N$ be the parameters' \textit{importances}. When training on task $k$, regularisation methods use the loss 
\[
\tilde{L}_k = L_k + c\cdot \sum_{i=1}^N \omega_i ^{(k-1)}\left(\theta_i - \theta^{(k-1)}_i\right)^2
\]
where $c>0$ is a hyperparameter. The first term $L_k$ is the standard (e.g.\ cross entropy) loss of task $k$. The second term ensures that the parameters do not move away too far from their previous values.
Usually, $\omega_i^{(k)} = \omega_i^{(k-1)} + \omega_i$, where $\omega_i$ is the importance for the most recently learned task $k$.
%How good a regularisation approach is, depends on how meaningful its importances are. Different estimates have been proposed and here we will understand their effectiveness and similarities.










\subsection{Review of EWC, MAS, SI and follow-ups}\label{sec:desc}
We describe the three main approaches to regularisation in continual learning and their follow-ups.

\textbf{Elastic Weight Consolidation} \citep{kirkpatrick2017} uses the diagonal of the Fisher Information as importance measure. It is evaluated at the end of training a given task. To define the \textit{Fisher Information Matrix} $F$, we omit the task index $k$ and simply consider a dataset $\mathcal{X}$. 
For each datapoint $X\in \mathcal{X}$ the network predicts a probability distribution $\mathbf{q}_X$ over the set of labels $L$, where we suppress dependence of $q_X$ on $\theta$ for simplicity of notation. We denote the predicted probability of class $y$ by $\textbf{q}_X(y)$ for each $y\in L$. 
Let us assume that we minimize the negative log-likelihood $\log \mathbf{q}_X(y)$ and write $g(X,y)=-\frac{\partial \log\textbf{q}_X(y)}{\partial \theta}$ for its gradient. 
Then the Fisher Information $F$ is given by
\begin{eqnarray}
F = 	 \mathbb{E}_{X\sim\mathcal{X}}	\mathbb{E}_ {y\sim \mathbf{q}_X} \left[g(X,y)g(X,y)^T
\right]
= 
\mathbb{E}_{X\sim \mathcal{X}}	\sum_{y \in L} \textbf{q}_X(y) \cdot g(X,y)g(X,y)^T
\label{fish}
\end{eqnarray}
Taking only the diagonal of $F$ means 
$\omega_i (\EWC)= \mathbb{E}_{X\sim \mathcal{X}}\EE_{y\sim \textbf{q}_X} \left[g_i(X,y)^2\right].$

The \textit{Empirical Fisher Information} replaces the expectation over $y\sim \textbf{q}_X$ by the (deterministic) label $y$ given by the labels of the dataset. We will also define the \textit{Predicted Fisher Information} as taking the maximum-likelihood predicted label, i.e.\ the argmax of $\textbf{q}_X(\cdot)$. When the network classifies images correctly and confidently, these three versions clearly become increasingly similar.
%Our empirical findings suggest that these different version of the Fisher Information can be used almost exchangeably, see appendix.  

%The Fisher Information is often used as a measure of parameter sensitivity and  
Under the assumption that the learned label distribution $\textbf{q}_X$ is the real label distributionthe Fisher equals the Hessian of the loss \citep{martens2014new, pascanu2013revisiting}. Its use for continual learning has a clean, bayesian, theoretical interpretation \citep{kirkpatrick2017, huszar2018}.


\textbf{Memory Aware Synapses} \citep{aljundi2018} heuristically argues that the sensitivity of the final layer with respect to a parameter should be used as the parameter's importance. This sensitivity is evaluated after training a given task. Denoting, as before, the final layer of learned probabilities by $\mathbf{q}_X$, this is implemented as (using a euclidean norm)
$$
\omega_i(\MAS) = \mathbb{E}_{X\sim \mathcal{X}}\left[  \left| \frac{\partial \|\textbf{q}_X\|^2}{\partial \theta_i} \right|\right],
$$
%where the norm is Euclidean.\footnote{The authors of MAS point out that their measure could also be applied in an unsupervised setting, where the last layer does not necessarily represent predicted labels.}

\textbf{Synaptic Intelligence} \citep{zenke2017} approximates the contribution of each parameter to the decrease in loss and uses this contribution as importance. To formalise the `contribution of a parameter', let us denote the parameters  at time $t$ by $\theta(t)$ and the loss by $L(t)$. If the parameters follow a smooth trajectory in parameter space, we can write the \textit{decrease} in loss from time $0$ to $T$ as
\begin{eqnarray}
L(0) - L(T) =  - \int_{\theta(0)}^{\theta(T)} \frac{\partial L(t)}{\partial \theta} \theta'(t)  dt  %\label{SI_first}
=  -\sum_{i=1}^N \int_{\theta_i(0)}^{\theta_i(T)} \frac{\partial L(t)}{\partial \theta_i} \theta_i'(t)  dt \label{def_contribution}. 
\end{eqnarray}
The $i$-th summand in (\ref{def_contribution}) can be interpreted as the contribution of parameter $\theta_i$ to the decrease in loss.
While we cannot evaluate the integral precisely, we can use a first order approximation to obtain the importances. 
To do so, we write $\Delta_i(t)=(\theta_i(t+1)-\theta_i(t))$ for an approximation of $\theta_i'(t) dt$ and get
\begin{eqnarray}\label{eq:def_SI}
\tilde{\omega_i}(\SI) =   \sum_{t=0}^{T-1} \frac{\partial L(t)}{\partial \theta_i} \cdot \Delta_i(t).
\end{eqnarray}
In addition, SI rescales its importances as follows\footnote{Note that the $\max(0,\cdot)$ is not part of the description in \citep{zenke2017}. However, we needed to include it to reproduce their results. A similar mechanism can be found in the official SI code.}
\begin{eqnarray}\label{eq:rescale}
\omega_i(\SI) = \frac{\max\left\{0, \tilde{\omega_i}(\SI)\right\}}{(\theta_i(T)-\theta_i(0))^2+\xi}.
\end{eqnarray}
%We empirically found that this normalisation has a very small (but positive effect). 


\citet{zenke2017} use additional assumptions, violated in practice, to theoretically justify this importance measure. One of the assumptions is using full batch gradient descent and we will show that this has an important effect. 



\textbf{Follow up work.}
Strictly speaking, we presented a version of EWC described in \citep{huszar2018} and tested in \citep{chaudhry2018, schwarz2018}. This version is theoretically more sound and was shown to perform better. Riemannian Walk \citep{chaudhry2018} is a combination of EWC and a `KL-rescaled' version of SI. Similar to EWC,  \cite{ritter2018} use the Fisher Information for regularisation, but rather than a diagonal approximation, finds a block diagonal approximation. 
%allowing to take layer-wise parameter interactions into account. While improving performance, this comes at the cost of a memory requirement of order $N\cdot K$ (where N is the number of parameters and K the number of tasks) which is enough memory to train and store separate networks for each task. 
In a similar vein, \cite{yin2020sola} use the full Hessian matrix for small networks. 































































\begin{table}[t]
	%\vskip -32pt
	\caption{\textbf{Summary of Regularisation Methods.} Algorithms SI, MAS, Fisher (EWC) are known methods; remaining algorithms are introduced here for detailed understanding that SI and MAS are closely related to Absolute Fisher, a natural variant of the Fisher Information.\\
		\textit{Details:}
		Algorithms on the left calculate importance `online' along the parameter trajectory during training. Algorithms on the right calculate importance at the end of training a task by going through (part of) the training set again. Thus, the sum is over timesteps $t$ (left) or datapoints $X$ (right). $N$ is the number of images over which is summed. All the algorithms on the left rescale their final importances as in equation \eqref{eq:rescale} for fair comparison.
		$\Delta(t)= \theta(t+1) - \theta(t)$ refers to the parameter update at time $t$, which depends on both the current task's loss and the auxiliary regularisation loss. Moreover, 
		$(g_t+\sigma_t)$ refers to the stochastic gradient estimate of the current task's loss (where $g_t$ is the full gradient and $\sigma_t$ the noise) given to the optimizer to update parameters. In contrast, $(g_t + \sigma_t')$ refers to an independent stochastic gradient estimate.
		For a datapoint $X$, $\textbf{q}_X$ denotes the predicted label distribution and 
		$g(X,y)$ refers to the gradient of the negative log-likelihood of $(X,y)$.
	}\label{table:overview}
	\iffalse
	\caption{\textbf{Overview of different algorithms and their importance measures for one task.} 
		Algorithms on the left calculate importance `online' along the parameter trajectory during training. Algorithms on the right calculate importance at the end of training a task by going through (part of) the training set again: The sum is over timesteps $t$ (left) or datapoints $X$ (right). $N$ is the number of images over which is summed. Note that all the algorithms on the left rescale their final importances as in \eqref{eq:rescale}.
		In all algorithms $\Delta(t)= \theta(t+1) - \theta(t)$ refers to the parameter update at time $t$, which depends on both the current task's loss and the regularisation loss. Moreover, 
		$(g_t+\sigma_t)$ refers to the stochastic gradient estimate of the current task's loss (where $g_t$ is the full gradient and $\sigma_t$ the noise) given to the optimizer (together with the regularisation loss) to calculate the parameter update. In contrast, $(g_t + \sigma_t')$ refers to an independent stochastic gradient estimate of the current task loss.
		For a datapoint $X$, $\textbf{q}_X$ denotes the predicted label distribution and 
		$g(X,y)$ refers to the gradient of the negative log-likelihood of $(X,y)$. }
	\fi
	%\vskip -0.5in
	\centering
	\begin{small}
		\begin{tabular}{ll|c|ll}
			\toprule
			\textbf{Name}  & \makecell{\textbf{Paramater} \\ \textbf{importance } $\mathbf{\omega(\cdot)}$}  &&\textbf{Name}  & \makecell{\textbf{Paramater} \\ \textbf{importance } $\mathbf{\omega(\cdot)}$}
			%&\makecell{\textbf{Normalisation} \\ $\omega(\cdot) \leftarrow \omega(\cdot) / (l^2+\epsilon )$ } 
			\\ \midrule
			SI &  $\displaystyle\sum_{t}^{} (g_t+\sigma_t)\Delta(t)$ && Fisher (EWC)  & $\displaystyle\frac1N\sum_X \EE_{y\sim \textbf{q}_X}\left[g(X,y)^2 \right] $ %&$\surd$ 
			\\
			%\midrule
			SIU (SI-Unbiased)  & $\displaystyle\sum_t (g_t+\sigma_t')\Delta(t)$ && AF (Absolute Fisher)  & $\displaystyle\frac1N\sum_X \EE_{y\sim \textbf{q}_X}\left[|g(X,y)| \right] $
			%&$\surd$
			\\
			%\midrule
			SIB (SI Bias-only)&  $\displaystyle\sum_t (\sigma_t- \sigma_t')\Delta(t)$  && MAS & $\displaystyle\frac1N\sum_X \left|\frac{\partial ||\textbf{q}_X||^2}{\partial \theta}\right| $
			%&$\surd$ 
			\\
			%	\midrule					
			OnAF (Online AF)  & $\displaystyle\sum_t |g_t+\sigma_t|$ && MASX (MAS-Max)   & $\displaystyle\frac1N\sum_X \left|\frac{\partial (\max \textbf{q}_X)^2}{\partial \theta}\right| $
			%&$\surd$ 
			\\ 
			\bottomrule
		\end{tabular}
	\end{small}
	\vskip -0.15in
\end{table}






==> ic/sections/X_04_theory.tex <==
\section{Theory \& Methods}
In this section we describe our theoretical results and design experiments to test our hypotheses,  focussing on Memory Aware Synapses (MAS) in Section \ref{sec:memory} and on Synaptic Intelligence (SI) in Section \ref{sec:synaptic}. The empirical results of our experiments will be presented in Section \ref{sec:experiments}. An overview of different algorithms described here can be found in Table \ref{table:overview}.

\begin{table}[t]
	%\vskip -0.1in
	\caption{\textbf{Summary of Regularisation Methods.} The three algorithms SI, MAS, Fisher (EWC) are the three known algorithms, which have inspired serveral follow ups. The other algorithms are introduced here in order to show that SI and MAS are closely related to Absolute Fisher, which is a natural variant of the Fisher Information.\\
		\textit{Details:}
		Algorithms on the left calculate importance `online' along the parameter trajectory during training. Algorithms on the right calculate importance at the end of training a task by going through (part of) the training set again. Thus, the sum is over timesteps $t$ (left) or datapoints $X$ (right). $N$ is the number of images over which is summed. Note that all the algorithms on the left rescale their final importances as in equation \eqref{eq:rescale}.
		$\Delta(t)= \theta(t+1) - \theta(t)$ refers to the parameter update at time $t$, which depends on both the current task's loss and the auxiliary regularisation loss. Moreover, 
		$(g_t+\sigma_t)$ refers to the stochastic gradient estimate of the current task's loss (where $g_t$ is the full gradient and $\sigma_t$ the noise) given to the optimizer to update parameters. In contrast, $(g_t + \sigma_t')$ refers to an independent stochastic gradient estimate.
		For a datapoint $X$, $\textbf{q}_X$ denotes the predicted label distribution and 
		$g(X,y)$ refers to the gradient of the negative log-likelihood of $(X,y)$.
	 }\label{table:overview}
	\iffalse
	\caption{\textbf{Overview of different algorithms and their importance measures for one task.} 
		Algorithms on the left calculate importance `online' along the parameter trajectory during training. Algorithms on the right calculate importance at the end of training a task by going through (part of) the training set again: The sum is over timesteps $t$ (left) or datapoints $X$ (right). $N$ is the number of images over which is summed. Note that all the algorithms on the left rescale their final importances as in equation \eqref{eq:rescale}.
		In all algorithms $\Delta(t)= \theta(t+1) - \theta(t)$ refers to the parameter update at time $t$, which depends on both the current task's loss and the regularisation loss. Moreover, 
		$(g_t+\sigma_t)$ refers to the stochastic gradient estimate of the current task's loss (where $g_t$ is the full gradient and $\sigma_t$ the noise) given to the optimizer (together with the regularisation loss) to calculate the parameter update. In contrast, $(g_t + \sigma_t')$ refers to an independent stochastic gradient estimate of the current task loss.
		For a datapoint $X$, $\textbf{q}_X$ denotes the predicted label distribution and 
		$g(X,y)$ refers to the gradient of the negative log-likelihood of $(X,y)$. }
	\fi
	%\vskip -0.5in
	\centering
	\begin{small}
		\begin{tabular}{ll|c|ll}
			\toprule
			\textbf{Name}  & \makecell{\textbf{Paramater} \\ \textbf{importance } $\mathbf{\omega(\cdot)}$}  &&\textbf{Name}  & \makecell{\textbf{Paramater} \\ \textbf{importance } $\mathbf{\omega(\cdot)}$}
			%&\makecell{\textbf{Normalisation} \\ $\omega(\cdot) \leftarrow \omega(\cdot) / (l^2+\epsilon )$ } 
			\\ \midrule
			SI &  $\displaystyle\sum_{t}^{} (g_t+\sigma_t)\Delta(t)$ && Fisher  & $\displaystyle\frac1N\sum_X \EE_{y\sim \textbf{q}_X}\left[g(X,y)^2 \right] $ %&$\surd$ 
			\\
			%\midrule
			SIU (SI-Unbiased)  & $\displaystyle\sum_t (g_t+\sigma_t')\Delta(t)$ && AF (Absolute Fisher)  & $\displaystyle\frac1N\sum_X \EE_{y\sim \textbf{q}_X}\left[|g(X,y)| \right] $
			%&$\surd$
			\\
			%\midrule
			SIB (SI Bias-only)&  $\displaystyle\sum_t (\sigma_t- \sigma_t')\Delta(t)$  && MAS & $\displaystyle\frac1N\sum_X \left|\frac{\partial ||\textbf{q}_X||^2}{\partial \theta}\right| $
			%&$\surd$ 
			\\
			%	\midrule					
			OnAF (Online AF)  & $\displaystyle\sum_t |g_t+\sigma_t|$ && MASX (MAS-Max)   & $\displaystyle\frac1N\sum_X \left|\frac{\partial (\max \textbf{q}_X)^2}{\partial \theta}\right| $
			%&$\surd$ 
			\\ 
			\bottomrule
		\end{tabular}
	\end{small}
	
	
	%\vskip -0.15in
\end{table}






\subsection{Memory Aware Synapses (MAS) and `Absolute Fisher Information'}\label{sec:memory}
We start by taking a closer look at the definition of the importances of MAS. We apply linearity of derivatives, the chain rule and write $y_0 = \argmax \mathbf{q}_X$ to obtain
\begin{eqnarray}\label{MAS1}
\frac{\partial \|  \textbf{q}_X \|^2}{\partial\theta} 
= 2\sum_{y\in Y} \textbf{q}_X(y) \frac{\partial \textbf{q}_X(y)}{\partial \theta}  
\approx 2 \textbf{q}_X(y_0)\frac{\partial \textbf{q}_X(y_0)}{\partial \theta} = 2 \textbf{q}^2_X(y_0)\frac{\partial \log \textbf{q}_X(y_0)}{\partial \theta}. %= 2 \textbf{q}^2_X(y_0) g(X,y_0)
\end{eqnarray}
Here we made the assumption that the sum is dominated by its maximum-likelihood label $y_0$, which should be the case if the network classifies its images confidently, i.e.\ $\textbf{q}(y_0)\gg \textbf{q}(y)$ for $y\neq y_0$. Recall that the importance is measured at the end of training, so that our assumption is justified  if the task has successfully been learned.
Using the same heuristic for the Fisher Information we obtain $$
\EE_{y\sim \textbf{q}_X}\left[g(X,y)^2\right] \approx \textbf{q}_X(	y_0) g(X,y_0)^2 = \textbf{q}_X(y_0) \left(\frac{\partial\log \textbf{q}_X(y_0)}{\partial\theta}\right)^2.
$$
Comparing this with \eqref{MAS1} makes the similarity between MAS and the Fisher Information apparent.
The only difference is that MAS has an additional factor of $2\textbf{q}_X(y_0)$ and that $g(X,y_0)$ is not squared.  
We therefore hypothesise that MAS is almost linearly dependent of the Absolute Fisher (AF), which is analogous to the Fisher Information, but takes absolute values of gradients rather than their squares, c.f.\ Table \ref{table:overview}. 

Our hypothesis is based on two assumptions: (a) The sum over the labels is dominated by its maximum likelihood label $y_0$, cf. equation \eqref{MAS1}. 
(b) We assume that the factor $2\textbf{q}_X(y_0)$ is roughly constant across most images $X$.

To check (a), we explicitly evaluate the term of the sum based on $y_0$ (and call this $\omega(\MASX)$, see Table \ref{table:overview}), and compare it to the entire sum (MASX vs MAS). See Figures \ref{figure:SI_scatter}A (top) and \ref{figure:correlations} (top) for strong empirical confirmations that the two measures are almost identical. 

 (b) is justified because at the end of training most images $X$ will have ${q}_X(y_0)\approx 1$. Note that even images with ${q}_X(y_0)=0.5$ deviate only by a factor of 2, and still lead to a large correlation between MAS and AF. As an empirical validation we check whether MASX and AF are linearly dependent.
Again, empirical evidence strongly supports this claim, see Figures \ref{figure:SI_scatter}A (middle\&bottom) and \ref{figure:correlations} (top). 






\subsection{Synaptic Intelligence (SI)}\label{sec:synaptic}
\subsubsection{Bias of Synaptic Intelligence}\label{bias}
To calculate $\omega(\SI)$, we need to calculate the product $p = \frac{\partial L(t)}{\partial \theta}\cdot\Delta(t)$ at each step $t$. Since evaluating the full gradient $\frac{\partial L(t)}{\partial \theta}$ is prohibitively expensive, SI \citep{zenke2017} uses a mini-batch. The resulting estimate is biased since the same mini-batch is used for the parameter update $\Delta(t)$ and the estimate of $\frac{\partial L(t)}{\partial \theta}$. 

We now give the calculations detailing the argument above.
For ease of exposition, let us assume that the network is optimized using vanilla SGD with learning rate $1$. 
%Very similar arguments apply to other optimizers. 
Given a mini-batch, denote its gradient estimate by $g+\sigma$, where $g=\frac{\partial L(t)}{\partial \theta}$ denotes the real gradient and $\sigma$ the mini-batch noise. With SGD the parameter update equals $\Delta(t) =  g+\sigma$. Thus, our product $p$ should be  
$p = g \cdot(g+\sigma).$ 
However, using $g+\sigma$, which was used for the parameter update, to estimate $\frac{\partial L(t)}{\partial \theta_i}$ results in 
$p_{biased} = (g+\sigma)^2.$ 
Thus, the gradient noise introduces a bias of
$\mathbb{E}[\sigma^2 +\sigma g] = \EE[\sigma^2].$

\paragraph{Unbiased Synaptic Intelligence.}
It is easy to design an unbiased estimate of $p$ by using two independent mini-batches to calculate the parameter update and to estimate $g$. This way we get $\Delta(t) =  g+\sigma$ and an estimate $g+\sigma'$ for $g$ from an independent mini-batch with independent noise $\sigma'$. We obtain
$
p_{unbiased} = (g+\sigma') \cdot (g+\sigma) 
$
which in expectation is equal to $p = g \cdot(g+\sigma).$
Based on this we define an unbiased importance measure
$$
\tilde{\omega_i}(\SIU) =  \sum_{t=0}^{T-1} (g_t+\sigma_t') \cdot \Delta(t). 
$$
%where the dash indicated that the gradient estimate is independent of the parameter update.

\paragraph{Bias-Only version of SI.}\label{bias_only}
To isolate the bias, we can simply take the difference between biased and unbiased estimate. Concretely, this gives a measure which only measures the bias of SI and is independent of the path integral, 
$$
\tilde{\omega_i}(\SIB) =   \sum_{t=0}^{T-1} ((g+\sigma)-(g+\sigma_t')) \cdot \Delta(t). 
$$ Observe that this estimate multiplies the parameter-update $\Delta(t)$ with nothing but stochastic gradient noise. From the perspective of SI, this should not be meaningful and have poor continual learning performance.


\paragraph{Which part dominates SI?}\label{exp:SI}
The approximations presented in equation (\ref{def_contribution}) imply that $L(0)-L(T)\approx\sum_i \tilde{\omega}_i(SI)$. Thus, comparing $\sum_i \tilde{\omega}_i$ for SI, SIU, SIB to $L(0)-L(T)$ measures how good the approximations are and shows whether SI is dominated by its bias, see Figure \ref{figure:summed_MNIST}. Further, comparing the continual learning performance of SI, SIU, SIB shows whether SI relies on the approximation of the path integral or its bias, see Table \ref{table:results}, Exp No 2.


\subsubsection{Synaptic Intelligence and Absolute Fisher Information}\label{sec:SI_FI}
In this section we will indicate the relation between the importance measure $\omega(\SI)$ and the Fisher Information.
Recall that $\omega(SI)$ is a sum over terms $\frac{\partial{L(t)}}{\partial \theta} \cdot \Delta(t)$, where $\Delta(t) = \theta(t+1) - \theta(t)$ is the parameter update at time $t$. Recall as well that both terms in this product, $\frac{\partial{L(t)}}{\partial \theta}$ as well as $\Delta(t)$, are computed/approximated using the same mini-batch and thus the have the same noise. 


For a precise understanding, we need to take into account how the optimizer uses stochastic gradients to update the parameters. The SI experiments (and ours) use the Adam optimizer \citep{kingma2014adam}. Given a stochastic gradient $g_t+\sigma_t$, 
it keeps a running average of the gradient $m_t = (1-\beta_1)(g_t+\sigma_t) + \beta_1 m_{t-1}$ as well as a running average of the squared gradients  $v_t = (1-\beta_2)(g_t+\sigma_t)^2 + \beta_2 v_{t-1}$. Ignoring some normalisation terms and the learning rate, the Adam parameter update is given by $\Delta(t) = m_t/(\sqrt{v_t} + \epsilon)$, where $\beta_1=0.9$ and $\beta_2 = 0.999$. Thus, 
\begin{eqnarray*}
	\frac{\partial L(t)}{\partial \theta} \Delta(t) = 
	%(g+\sigma)\cdot \frac{(1-\beta_1)(g+\sigma) + \beta_1 m_{t-1}}{\sqrt{v_t} + \epsilon} \\
	\frac{(1-\beta_1)(g_t+\sigma_t)^2}{{\sqrt{v_t} + \epsilon}} + \frac{\beta_1(g_t+\sigma_t)m_{t-1}}{{\sqrt{v_t} + \epsilon}}.
\end{eqnarray*}
Assuming that the noise $\sigma_t$ is considerably bigger than the gradient $g_t$  we obtain
\begin{eqnarray}\label{eq:noise}
\frac{\partial L(t)}{\partial \theta}\Delta(t) 
%=  (1-\beta_1) \frac{(g_t+\sigma_t)^2}{{\sqrt{v_t} + \epsilon}} + \beta_1\frac{g_t()}{{\sqrt{v_t} + \epsilon}}   
\approx (1-\beta_1)\frac{(g_t+\sigma_t)^2}{{\sqrt{v_t} + \epsilon}} \label{eq:main_SI_bias} %\nonumber
\end{eqnarray}
The assumption made here is $(1-\beta_1)\sigma_t^2\gg \beta_1 m_{t-1}g_t$ (we ignore the term $\sigma_t m_{t-1}$ since $\EE[\sigma_t m_{t-1}]=0$ and since we average SI over many time steps). This assumption is supported strongly by Figure \ref{figure:summed_MNIST}, where the difference between green (SI) and blue (SIU) line is caused precisely by $(1-\beta_1)\sigma^2$, see \ref{sec:calc_bias} for full details. We also refer to \citep{lan2019} and Figures \ref{figure:noise}, \ref{figure:noise_cdf} and \ref{figure:summed_cifar_all}, \ref{figure:summed_mnist_all}  for more evidence that the noise is considerably bigger than the gradient.

%are summed over time. 
%In addition, the denominator $\sqrt{v_t}$ changes only slowly (since $\beta_2=0.999$) 
%and is roughly equal to $\sqrt{\EE[(g_t+\sigma_t)^2]}$ across time. Therefore, 

Next, we consider $v_t$. It is a slowly moving exponential average of $(g_t+\sigma_t)^2$ and will therefore be approximately $\EE[(g_t+\sigma_t)^2]$. It is thus reasonable to expect that $\sqrt{v_t}$ is roughly proportional to $|g_t+\sigma_t|$. This clearly does not hold for all possible distributions of $g_t+\sigma_t$, but is unlikely to be violated by non adversarially chosen, realistic distributions. 
With \eqref{eq:noise} and $\sqrt{v_t}\appropto |g_t+\sigma_t|$ we arrive at 
\begin{eqnarray}\label{eq:SI-OnAF}
	\tilde{\omega}(SI) =\sum_t \frac{\partial L(t)}{\partial \theta}\Delta(t)\approx (1-\beta_1)\sum_t \frac{(g_t+\sigma_t)^2 }{\sqrt{v_t}} 
	%\propto \frac{\EE[(g_t+\sigma_t)^2]}{\sqrt{\EE[(g_t+\sigma_t)^2]}}
	\appropto \sum_t |g_t+\sigma_t|.
\end{eqnarray}

\iffalse
In SI, %the products 
$\frac{\partial{L(t)}}{\partial \theta} \cdot \Delta(t)$ is summed over time.
Moreover, $v_t$ is roughly  equal to $\EE[(g_t+\sigma_t)^2]$. Thus,
\begin{eqnarray*}
	\tilde{\omega}(SI) \approx (1-\beta_1)\sum_t \frac{(g_t+\sigma_t)^2 }{\sqrt{\EE[(g_t+\sigma_t)^2]}} 
	%\propto \frac{\EE[(g_t+\sigma_t)^2]}{\sqrt{\EE[(g_t+\sigma_t)^2]}}
	\appropto \sum_t |g_t+\sigma_t|.
\end{eqnarray*}
The last approximation assumes that $\sqrt{\EE[(g_t+\sigma_t)^2]}$ is approximately proportional to the magnitude $|g_t+\sigma_t|$ of a typical gradient, which seems rather plausible in a non-adversarial setting but is of course not true for all distributions of $g_t+\sigma_t$.
\fi
An alternative way to arrive at \eqref{eq:SI-OnAF} is following the analysis of \cite{balles2018dissecting}, who show that the update of Adam is mostly given by the sign of the moment $m_t$.
Our resulting approximation $\tilde{\omega}(SI)\appropto \sum_t |g_t+\sigma_t|$ is very similar to the (Empirical) Absolute Fisher. The only differences are (a) the gradient in $\tilde{\omega}(SI)$ is evaluated in mini-batches rather than on single images; (b) the sum is taken `online' along the parameter trajectory rather than at the final point of the trajectory. (a) does not have a large effect %(other than rescaling by the batch size)
when $\sigma_t\gg g_t$ (as detailed in \ref{sec:calc_batch}) which we have seen to be the case.
The influence of (b) is hard to quantify and depends on how much the gradients change along the parameter trajectory.
To capture this difference, we define the Online Absolute Fisher as 
$
\tilde{\omega} (\OnAF) = \sum_t |g+\sigma_t|
$
and empirically test how similar %$\tilde{\omega}(SI), \tilde{\omega}(\OnAF)$ as well as 
$\tilde{\omega}(\OnAF)$ and $\tilde{\omega}(\AF)$ are. The fact that Adam usually works well with $\beta_2=0.999$ suggests that the second moment of the gradient and thus OnAF change very slowly in many settings, indicating that OnAF and AF are often and robustly similar.

Our heuristics suggest that $\tilde{\omega}(\SI)$ and $\tilde{\omega}(\OnAF)$ are very similar. If in addition, we empirically see that $\tilde{\omega}(\OnAF)$ and $\tilde{\omega}(\AF)$ are similar, then SI approximates AF, a rescaling of the Fisher.  Figures \ref{figure:SI_scatter}B and \ref{figure:correlations}  empirically confirm both parts of this hypothesis. 


We emphasise that our derivation above assumes that the parameter update $\Delta(t)$ is given by the gradients of the current task and ignores influence of regularisation on parameter updates. The latter will change update direction and momentum of the optimizer. Thus, strong regularisation will make the relation between SI and OnAF noisy, but not abolish it. 
See Fig \ref{figure:correlations} (middle row) and Appendix \ref{sec:effect_reg_SI} for various confirmations hereof.% for controls. %experiments.%showing that SI, SIB are more related to AF than SIU (and more effective at continual learning).




\begin{figure}[t]
	\begin{center}
		\begin{subfigure}{0.52\textwidth}
			%\vskip 0.1in
			\centerline{\includegraphics[width=\textwidth]{../figures/summed_contributions_mnist.png}}
			\vskip -0.05in
			\caption{}
			\label{figure:summed_MNIST}
		\end{subfigure}
		\begin{subfigure}{0.45\textwidth}
			\centerline{\includegraphics[width=\textwidth]{../figures/correlations_MAS.png}}
			\vskip -0.05in
			\centerline{\includegraphics[width=\textwidth]{../figures/correlations_SI_MAS.png}}
			\vskip -0.05in
			\caption{}
			\label{figure:correlations}
		\end{subfigure}
		\vskip -0.1in
		\caption{
			\textbf{(a)} \textbf{Summed importances} $\sum_i \tilde{\omega}_i$ for Permuted-MNIST.  
			\textbf{(b)} \textbf{Pearson correlations of importances for all tasks.} Dashed lines represent CIFAR, solid lines MNIST. Error bars are stds for 4 runs. `AF' is an estimates the Absolute Fisher with 30000 (MNIST) resp.\ 5000 (CIFAR) images. `AF\_small', `MAS' and `MASX' use 1000 resp.\ 500 images.
		}
	\end{center}
	\vskip -0.2in
\end{figure}



==> ic/sections/X_05_experiments.tex <==
\section{Experiments}\label{sec:experiments}
In this section we empirically test our three main hypotheses:
\begin{enumerate}
	\item Does Memory Aware Synapses approximate the Absolute Fisher as derived in Sec \ref{sec:memory}?
	\item Which part of the importance $\tilde{\omega}(SI)$ of Synaptic Intelligence, the bias or the unbiased contribution, explains its effectiveness, see Section \ref{bias}?
	\item Does $\tilde{\omega}(SI)$ correlate strongly with  the Absolute Fisher as indicated in Sec \ref{sec:SI_FI}?
\end{enumerate}
%Our affirmative answers to question 1.\ and 3.\ suggest that both Memory Aware Synapses (MAS) and Synaptic Intelligence (SI) work because they approximate a rescaled version of the Fisher Information, which is a somewhat sound theoretical explanation for their effectiveness. At the same time, it raises the question whether the rescaled version (i.e.\ Absolute Fisher) or the original Fisher Information is more effective, which is the last question we investigate.  



\subsection{Experimental Setup}
Our experiments closely follow \citep{zenke2017}. We use the \textbf{Permuted MNIST} \citep{goodfellow2013} benchmark with 10 tasks, a fully connected ReLU architecture and a single output-head (`domain incremental' setting, c.f.\ \citep{hsu2018,van2019}) and the \textbf{Split CIFAR 10/100} benchmark with the keras default CNN and a multi-head output (`task incremental').  
Following \citep{swaroop2019}, but unlike \citep{zenke2017}, we re-initialise model variables (fully connected layers, etc.) after each task and usually find better performance in our hyperparameter searchers.
We defer further experimental details to the Appendix \ref{sec:exp_detail}. Code is available on github\footnote{\url{https://github.com/freedbee/continual_regularisation}}.

%How similar AF and OnAF are depends on how quickly the gradient changes along the parameter trajectory. 
\begin{figure}[t]
	\vskip -8pt
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/MAS_MASX_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure}
	\hspace{6pt}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_OnAF_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/OnAF_AF_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_AF_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure} 
	
	\vskip -0.2in
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/MAS_AF_scatter_CIFAR_task_1.png}}
		\end{center}
	\end{subfigure}
	\hspace{6pt}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_OnAF_int_CIFAR_task_6.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/OnAF_AF_int_CIFAR_task_6.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_AF_int_CIFAR_task_6.png}}
		\end{center}
	\end{subfigure} 
	\vskip -0.2in
	
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/MAS_AF_int_MNIST_task_5.png}}
		\end{center}
	\end{subfigure}
	\hspace{6pt}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_OnAF_int_MNIST_task_5.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/OnAF_AF_big_int_MNIST_task_5.png}}
		\end{center}
	\end{subfigure}
	\begin{subfigure}{0.24\textwidth}
		\begin{center}
			\centerline{\includegraphics[width=\textwidth]{../figures/SI_AF_big_int_MNIST_task_5.png}}
		\end{center}
	\end{subfigure} 
	\vskip -0.3in
	\caption{
		\textbf{Scatter- and Intensity plots for pairs of importance measures.} 
		$r$ denotes the Pearson correlation.
		\textit{Scatter Plots (blue):} Each point in the scatter plot corresponds to one weight of the net. A straight line through the origin corresponds to two importances measures being multiples of each other. 
		\textit{Intensity Plots (gray scale):} Show data analogous to scatter plots, but are normalised for better visualisation. See \ref{sec:intensity} for details and Fig \ref{fig:scatter_app} for same data with only scatter/intensity plots.
		\textbf{(A)} Comparison between MAS, MASX, AF. 
		\textbf{(B)} Comparison between SI, OnAF, AF on first task of CIFAR (top),  last task of CIFAR (middle) and `middle' task of MNIST (bottom). See Fig \ref{figure:correlations} for data on all tasks.}
	\label{figure:SI_scatter}
	\vskip -0.1in
\end{figure}

%and we will assess empirically how strong the correlation between OnAF and AF as well as whether our heuristics 

%We note that our derivation for the similarity of SI and OnAF relies on the approximation made in \eqref{eq:main_SI_bias}, which is due to the bias of SI.

%We empirically assess the correlation between $\tilde{\omega}(SI)$ and $\tilde{\omega}(\OnAF)$ as well as the difference between SI and Absolute Fisher in Figure \ref{figure:SI_scatter}.





\subsection{Results}
\paragraph{MAS and Absolute Fisher.}
Our first objective is to test whether MAS and Absolute Fisher are related. To this end we  calculate $\omega(\MAS)$, $\omega(\MASX)$, $\omega(\AF)$  and show scatter plots of these values in Figure \ref{figure:SI_scatter} \textbf{(A)}. We  find that they are almost identical. Figure \ref{figure:correlations} shows equally strong correlations on the other tasks and datasets, presenting strong evidence for our heuristics.
We also evaluated continual learning algorithms based on $\omega(\MAS)$, $\omega(\MASX),$ $\omega(\AF)$ and found very similar results, Table see \ref{table:results}, Exp No 1, providing further evidence that our mathematical derivations hold.

\paragraph{Why does SI work?}
To understand how large the bias of SI is, we track the sum $\sum_{i} \tilde{\omega}_i$ of importances for SI and its unbiased version SIU. As a control we 
include the decrease of the loss $L(0)-L(T)$ which the path-integral (c.f.\ equation (\ref{def_contribution})) approximates, as well as an first order approximation of the path-integral without relying on stochastic gradient estimates (computing the full training set gradient at each step). The results are portrayed in Figure \ref{figure:summed_MNIST}. They indicate that (1) the bias is 5-6 times larger than the unbiased part;  (2) using an unbiased gradient estimate and using the entire training set gradient gives almost identical values of $\sum_i\omega_i$ supporting the validity of the unbiased estimator; (3) even the unbiased first order approximation of the path integral overestimates the decrease in loss. This is consistent with previous empirical studies showing that the loss has positive curvature \citep{jastrzebski2018relation, lan2019}.  See Figures \ref{figure:summed_cifar_all}, \ref{figure:summed_mnist_all} for similar results on CIFAR and other MNIST tasks.

We have seen that the SI's bias is considerably larger than its unbiased component. This does not fully explain which of these parts is more essential for continual learning. We therefore run continual learning algorithms based on SI, its unbiased version (SIU) as well as a version which isolates the bias (SIB). The results are shown in Table \ref{table:results}, Exp No.\ 2. SIU consistently has worse performance than SI and SIB has the same or slightly better performance than SI. From SI's perspective this is rather surprising and is convincing evidence that SI's continual learning capability is due to its bias.






\paragraph{Is SI related to Absolute Fisher?} Our main assumption in relating SI to Online Absolute Fisher (OnAF) was that the contribution of the  noise (bias) to SI is bigger than its unbiased part, c.f.\ equation \eqref{eq:noise}. We have already seen strong evidence that this is the case (Figure \ref{figure:summed_MNIST}). Therefore it may be expected that OnAF and SI do have significant correlations: On all tasks of MNIST and the first task of CIFAR, SI and OnAF have (Pearson) correlations $>0.93$; on tasks 2-6 of CIFAR we find weaker, but significant correlations around 0.5, see Figures \ref{figure:SI_scatter}, \ref{figure:correlations}. This weaker correlation on CIFAR tasks 2-6 is well explained by regularisation, see \ref{sec:SI_FI} and Appendix \ref{sec:effect_reg_SI} for two control experiments. 

We also find that OnAF and AF are surprisingly similar, thus closely relating SI and AF (Figures \ref{figure:SI_scatter}, \ref{figure:correlations}) supporting our hypotheses.\footnote{ We check in \ref{sec:training_time} that similarity of AF, OnAF does not depend on how long the networks are trained and show control correlations between SIU, SIB and (On)AF in \ref{sec:controls}, further supporting our claim, that continual learning performance is explained by similarity to AF.}
We also evaluate the corresponding continual learning algorithms SI, OnAF and AF, see Table \ref{table:results}, Exp 3. The results are very similar, indicating that SI, like MAS, works because it approximates a rescaled version of the Fisher Information. %We believe that the slight gap between performance of SI, OnAF as compared to AF on CIFAR is due to the normalisation of SI and OnAF given in equation (\ref{eq:rescale}), see appendix for an ablation experiment.





\paragraph{Is Absolute or Real Fisher better for continual learning?}
We have seen evidence that both MAS and SI rely on estimating a rescaled Fisher Information. This raises the questions whether a rescaled version of the Fisher or the Fisher itself are more effective for continual learning. To answer this, we compare MAS, AF  and EWC, since these methods all evaluate the importance at the end of training. 
The results are shown in Figure \ref{table:results}, Exp 4. All algorithms perform similarly, only the difference between MAS and EWC on CIFAR is significant ($p=0.04$, t-test, not corrected for multiple comparisons). Which algorithm performs best may well depend on hyperparameters and the precise training set-up.

%We find, maybe surprisingly, that on both continual learning tasks P-MNIST, and CIFAR 10/100 the rescaled, Absolute Fisher has slightly better performance. However, we can not exclude the possibility that this observation is data-set dependent.










\begin{table}[t]
	%\vskip -12pt
	\caption{\textbf{Test accuracies on Permuted-MNIST and Split CIFAR 10/100.} 
		Algorithms are grouped by experiment as indicated in main text.
		Reported results are mean and standard deviation over 3 resp. 10 runs for P-MNIST resp.\ CIFAR 10/100. 
	}
	\label{table:results}
	\vskip -0.2in
	\begin{center}
		%\vskip -0.2in
		\begin{small}
			%\vskip -0.1in
			\begin{sc}
				%\vskip -0.1in
				\begin{tabular}{cccc|c|cccc}
					\toprule
					\textbf{No.} & \textbf{Algo.} & \textbf{P-MNIST} & \textbf{CIFAR} & &\textbf{No.} & \textbf{Algo.} & \textbf{P-MNIST} & \textbf{CIFAR} \\
					\midrule
					\multirow{3}*{1}
					&  $\MAS$ & 97.3 $\pm$ 0.1& 73.7 $\pm$ 0.5 & &\multirow{3}*{3} & $\SI$ & 97.2 $\pm$ 0.1& 74.4 $\pm$ 0.5\\
					& $\MASX$ & 97.4 $\pm$ 0.2& 73.7 $\pm$ 0.2 &
					&& $\OnAF$& 97.3 $\pm$ 0.1&    74.4 $\pm$ 0.6 \\ 
					& $\AF$ & 97.4 $\pm$ 0.1& 73.4 $\pm$ 0.4&
					&& $\AF$ & 97.4 $\pm$ 0.1& 73.4 $\pm$ 0.4\\ 
					\midrule
					\multirow{3}*{2}
					& $\SI$ & 97.2 $\pm$ 0.1& 74.4 $\pm$ 0.5& 
					&\multirow{3}*{4} 
					& $\EWC$ & 97.2 $\pm$ 0.2& 73.1 $\pm$ 0.7 \\
					& $\SIU$ & 96.3 $\pm$ 0.1& 72.5 $\pm$ 0.8& 
					&&   $\MAS$ & 97.3 $\pm$ 0.1& 73.7 $\pm$ 0.5    \\
					& $\SIB$ & 97.2 $\pm$ 0.1& 75.1 $\pm$ 0.4&
					&& $\AF$ & 97.4 $\pm$ 0.1& 73.4 $\pm$ 0.4 \\
					\bottomrule
				\end{tabular}
			\end{sc}
		\end{small}
	\end{center}
	\vskip -0.3in
\end{table}









==> ic/sections/X_06_discussion.tex <==
\section{Discussion}\label{sec:rel}
We have investigated regularisation approaches for continual learning, which are the method of choice for continual learning without replaying old data or expanding the model. We have provided strong theoretical and experimental evidence that the three most influential methods in this domain are surprisingly similar. This does not only unify these three methods, but also their many follow ups. Additionally, relating SI and MAS to the Fisher Information has the benefit of putting these algorithms on a solid theoretical underpinning.  \citet{kirkpatrick2017, huszar2018} give a theoretical, bayesian explanation of why the Fisher Information, combined with a quadratic weight penalty is a principled approach to continual learning and recently, \citet{yin2020sola} provided theoretical guarantees as well as a frequentist interpretation of this approach. Our results extend these insights to all MAS- and SI-based algorithms. Moreover, our theoretical derivations imply that the findings presented here are much more robust than mere empirical observations of correlations.

A limitation of our theoretical results is that we do not precisely quantify the differences between SI, MAS and the Absolute Fisher. This would require precise knowledge of the gradient and noise distribution (to handle equations \eqref{MAS1}, \eqref{eq:SI-OnAF})	and the Hessian of the loss (to quantify the difference between OnAF and AF). Such knowledge is currently out of reach for deep neural networks. We therefore chose to present approximations, rather than proving theorems based on unrealistically strong assumptions. We found this to more effectively communicate our main findings.  

Our thorough analysis led to several new insights and algorithms. Among other things, it shows that: our algorithm OnAF is a more theoretically grounded version of SI; our (predictive) AF algorithm is more grounded than MAS; the Fisher Information can be calculated in mini-batches (c.f.\ our theoretical analysis \ref{sec:calc_batch} and the empirical correlation of OnAF with AF) offering large computational speed-ups over processing each training image individually (Figure \ref{figure:time}). Moreover, our algorithm SIU opens up the possibility to apply the (non continual learning related) algorithm LCA \citep{lan2019}) to larger datasets and architectures.

Finally, we hope that more future work will focus on unifying and explaining the ever growing body of continual learning literature, advancing our understanding of these methods and allowing to discover new, efficient algorithms.

 


\iffalse
We have investigated regularisation approaches for continual learning and more specifically, how these methods assess parameter importance. We have provided strong theoretical and experimental evidence that the three most influential methods in this domain are inherently similar. Our results are based on theoretical approximations and thorough empirical checks of these approximations. A limitation of our theoretical results is that we do not precisely quantify the differences between SI, MAS and the Absolute Fisher. This would require precise knowledge of the gradient and noise distribution (to handle equations \ref{MAS1}, \ref{eq:SI-OnAF})	and the Hessian of the loss  (to quantify the difference between OnAF and AF). Such knowledge is currently out of reach for deep neural networks. We therefore chose to present heuristics, rather than proving theorems based on unrealistically strong assumptions. We found this more instructive and to more effectively communicate our main insights.

From a theoretical viewpoint, our results unify many proposed algorithms. On top of that, relating SI and MAS to the Fisher Information has the benefit of putting these algorithms on a solid theoretical underpinning.  \cite{kirkpatrick2017, huszar2018} give a theoretical, bayesian explanation of why the Fisher Information, combined with a quadratic weight penalty is a principled approach to continual learning and recently, \cite{yin2020sola} provided theoretical guarantees for this approach.

From a practical viewpoint, our insights explain under which circumstances MAS and SI provide good approximations of the Absolute Fisher and are thus likely to perform well. For example, SI's performances should be expected to decrease with increasing batch-size as this diminishes its bias, which we showed to explain its performance. Similarly, we can see (theoretically and empirically) that the magnitude of SI importances depends on the training duration of a given task. This could very well explain why \cite{de2019continual} observe that SI is more sensitive to task-ordering than EWC and MAS.  We note that using a normalised version of OnAF could easily mitigate this problem. Likewise, the choice of optimizer, learning rate schedule, initialisation will impact SI all of which is accounted for by our results.

In addition, we point to a non-continual learning related implication of our analysis: The core idea of SI -- measuring parameter contribution to the decrease in loss -- was recently used to gain insights into the training process of neural networks by \cite{lan2019}. The authors found the SI-measure to overestimate this contribution, which is explained by the bias we described. They resorted to evaluating the full batch gradient at each update step during training, resulting in a computationally expensive algorithm. Our unbiased approximation, SIU, provides a much cheaper approximation of this quantity and allows testing their ideas on larger datasets and networks.

Finally, we hope that our contribution helps to direct attention towards understanding and unifying existing approaches. We believe this to be an important step for developing truly new and effective algorithms.
\fi

	
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	
	
\iffalse	
We have focused on regularisation approaches for continual learning and more specifically, how these methods assess parameter importance. We investigated three different importance measures proposed in the literature, namely Elastic Weight Consolidation, Synaptic Intelligence and Memory Aware Synapses. For standard (non-bayesian) neural networks these are (to the best of our knowledge) the only approaches to regularisation based continual learning. Other regularisation-related work directly relies on one of these algorithms or combinations of them \citep{kirkpatrick2017, zenke2017, aljundi2018, aljundi2019task, schwarz2018, ritter2018, chaudhry2018, huszar2018}. 
Originally, all three methods were motivated rather differently and suggested seemingly orthogonal importance measures. However, we gave heuristic mathematical derivations indicating that all methods nevertheless -- and somewhat accidentally -- are very closely related to the Fisher Information. We thoroughly checked the assumptions underlying our heuristics in realistic, standard continual learning set-ups and found convincing empirical support for our claims.\footnote{The complexity of these set-ups and our limited understanding of neural networks in general mean that precise mathematical theorems quantifying when which methods are how similar are currently out of reach. We therefore believe that our simple, clear heuristics are more meaningful and instructive than theorems relying on unrealistic assumptions or only treating toy examples.}


On the one hand, our work unifies regularisation approaches proposed so far and highlights unexpected similarities. Our mathematical derivations do not only explain some surprising results, but also imply that our findings are more robust than merely observing empirical correlations. %We also hope that our work can guide developing future regularisation methods into new directions.


%On the one hand, this gives a theoretical justification for  MAS' and SI's effectiveness. This is interesting not only from a theoretical perspective but for anybody applying or comparing to regularisation approaches, as it explains in which settings these algorithms are guaranteed to work or likely to fail. Let's give two concrete examples: SI should be expected to have worse performance with large batch sizes as it relies on its bias, which is due to gradient noise. MAS' performance might well degrade when the net is not trained too long and inputs are not classified confidently enough as this weakens its relation to the Fisher Information. This may also apply for long sequences of tasks, when it gets increasingly hard to classify new images confidently. Further, our work is relevant for developing new regularisation methods as it shows which kinds of algorithms are already well explored.

On the other hand, our findings can have immediate practical consequences, as they help explain which algorithms are likely to work in which setting. There are several situations, in which we can make grounded predictions on the relative performance of MAS, SI and EWC. To be concrete, we exhibit how our insights may explain empirical observations presented in \citep{de2019continual}, which is an extensive comparative study of continual learning algorithms. (1) \citep{de2019continual} finds that SI is sensitive to task-ordering when dataset sizes are imbalanced - namely, when small datasets are learned first SI overfits more. When training for a fixed number of epochs, small datasets will have small SI importances (since its biased sum contains few terms, independent of the path-integral) so that the net is subsequently less regularised and prone to overfit. (2) \citep{de2019continual} notes that EWC suffers from having many weights with small importances and performs worse than MAS. Note that relatively, MAS' (Absolute Fisher) rescaling makes small importances much bigger, explaining why it alleviates the small-importance problem. (3) \citep{de2019continual} reports bad performance of SI %(compared to MAS, EWC) 
in various settings. This may be due to learning rate decay, which gives more weight to early terms in SI's running sum. This makes the sum less related to the Fisher at the end of training, causing worse performance of SI. We note that (1) and (3) could be fixed by replacing SI by a normalised version of OnAF. We leave testing these hypoteheses to future work and hope that our insights help developing, testing and improving regularisation methods.

%On the other hand, our work unifies regularisation approaches proposed so far and highlights unexpected similarities. Our mathematical derivations do not only explain some surprising results, but also imply that our findings are more robust than merely observing empirical correlations. 
%They shed light on the inner workings of these algorithms.




%On the one hand, this gives a theoretical justification for  MAS' and SI's effectiveness. This is interesting not only from a theoretical perspective but for anybody applying or comparing to regularisation approaches, as it explains in which settings these algorithms are guaranteed to work or likely to fail. Let's give two concrete examples: SI should be expected to have worse performance with large batch sizes as it relies on its bias, which is due to gradient noise. MAS' performance might well degrade when the net is not trained too long and inputs are not classified confidently enough as this weakens its relation to the Fisher Information. This may also apply for long sequences of tasks, when it gets increasingly hard to classify new images confidently. Further, our work is relevant for developing new regularisation methods as it shows which kinds of algorithms are already well explored.

%On the other hand, our work unifies regularisation approaches proposed so far and highlights unexpected similarities. Our mathematical derivations do not only explain some surprising results, but also imply that our findings are more robust than merely observing empirical correlations. 
%They shed light on the inner workings of these algorithms.
\acks{
I would like to thank Xun Zou, Angelika Steger, Florian Meier, Kalina Petrova and Asier Mujika for many helpful discussions and valuable feedback on this manuscript. I am also thankful for AM's technical advice and the Felix Weissenberger Foundation's ongoing support. }

\fi


==> ic/sections/X_A_MAS-AF.tex <==
\section{Experimental Setup}
On top of theoretical derivations, the following sections contain experiments on standard continual learning benchmarks. Here, we outline our setup, see Appendix \ref{sec:exp_detail} for full details. 
We closely follow SI's setting \citep{zenke2017}: In domain-incremental \textbf{Permuted MNIST} \citep{goodfellow2013} each of 10 tasks consists of a random (but fixed) pixel-permutation of MNIST  and a \textbf{fully connected ReLU network} is used. The task-incremental \textbf{Split CIFAR 10/100} benchmark \citep{zenke2017} consists of six 10-way classification tasks, the first is CIFAR 10, and the other ones are extracted from CIFAR 100. The \textbf{keras default} CIFAR 10 \textbf{convolutional architecture} (with dropout and max-pooling) is used.   
The only difference to the setup of \citet{zenke2017} is that like \citet{swaroop2019}, we usually re-initialise the network weights after each task, observing performance improvements.
Code is available on github. %\footnote{\url{https://github.com/freedbee/continual_regularisation}}. 
For brevity, we sometimes only show plots based on one benchmark. The analogous plot based on the other benchmark can then be found in the appendix.

\section{Memory Aware Synapses (MAS) approximates Absolute Fisher}
Here, we explain why -- despite it's different motivation -- MAS is almost linearly dependent of the Absolute Fisher. We first present our theoretical reasoning and then carry out careful empirical confirmations of our derivation. 





\subsection{Theoretical Relation of MAS and Absolute Fisher}
We start by taking a closer look at the definition of the importances of MAS. We apply linearity of derivatives, the chain rule and write $y_0 = \argmax \mathbf{q}_X$ to obtain
\begin{align}\label{MAS1}
\textbf{MAS:}&\quad \frac{\partial \|  \textbf{q}_X \|^2}{\partial\theta} 
= 2\sum_{y\in Y} \textbf{q}_X(y) \frac{\partial \textbf{q}_X(y)}{\partial \theta}  
\approx 2 \textbf{q}_X(y_0)\frac{\partial \textbf{q}_X(y_0)}{\partial \theta} =2 \textbf{q}^2_X(y_0)\frac{\partial \log \textbf{q}_X(y_0)}{\partial \theta}. %= 2 \textbf{q}^2_X(y_0) g(X,y_0)
\intertext{Here we made the assumption that the sum is dominated by its maximum-likelihood label $y_0$, which should be the case if the network classifies its images confidently, i.e.\ $\textbf{q}(y_0)\gg \textbf{q}(y)$ for $y\neq y_0$. Recall that the importance is measured at the end of training, so that our assumption is justified  if the task has successfully been learned.
Using the same heuristic for the Fisher Information we obtain %(akin to the \textit{Predictive Fisher})
}
\textbf{Fisher:}&\quad \EE_{y\sim \textbf{q}_X}\left[g(X,y)^2\right] \approx \textbf{q}_X(	y_0) g(X,y_0)^2 = \textbf{q}_X(y_0) \left(\frac{\partial\log \textbf{q}_X(y_0)}{\partial\theta}\right)^2.
\end{align}
Comparing this with \eqref{MAS1} makes the similarity between MAS and the Fisher apparent.
We hypothesise that MAS is almost linearly dependent of the Absolute Fisher (AF), which is analogous to the Fisher Information, but takes absolute values of gradients rather than their squares, c.f.\ Table \ref{table:overview}. 

\subsection{Empirical Relation of MAS and Absolute Fisher}
Our theoretical derivation relied on two approximations, which we now explicitly check.

\textbf{Max-Likeilhood Approximation}
 First, in \eqref{MAS1} we assumed that sum over the labels is dominated by its maximum likelihood label $y_0$. To assess the validity of this, we directly compare the entire sum (MAS) with the part only using the max-likelihood label (MAS-MAX). 
 %This directly compares LHS to RHS of \eqref{MAS1}. 
 The results in Figure \ref{figure:MAS} show scatter plots and a summary of the pearson correlations between MAS and MAS-MAX on each task. On P-MNIST the correlations range from 0.95 to 0.99, on CIFAR they are always above 0.99. This is very strong support for MAS and MAS-MAX being nearly equal as hypothesised.
 
 \textbf{Absolute Fisher Approximation}
 Second, we hypothesised that the factor $2\textbf{q}_X(y_0)$ distinguishing MAS-MAX and Absolute Fisher is roughly constant. We note that even if  $\textbf{q}_X(y_0)$ varied between 0.5 (rather inconfident prediction) and 1.0 (absolutely confident), the two measures would have large correlations. The data in Figure \ref{figure:MAS} show that we are far above this pessimistic regime with correlations between MAS-MAX and AF always above 0.98, showing that MAS-MAX indeed approximates AF.
 The data also shows that the resulting correlation between MAS and AF is large (between 0.9-0.97 on MNIST, >0.99 on CIFAR), confirming that MAS is an approximation of AF. 
 
 \textbf{Continual Learning Performance Experiment}
 As an additional check of our hypothesis, we implemented continual learning algorithms based on MAS, MASX and AF and compared their performances. The results in Table \ref{table:results}(1) show that the algorithms are nearly indistinguishable, further supporting the claim that MAS is effective because it approximates the Absolute Fisher.
 
 
 
 
 
 
 
 
 \begin{table}[t]
 	\vskip -12pt
 	\caption{\textbf{Test accuracies on Permuted-MNIST and Split CIFAR 10/100.} 
 		%Algorithms are grouped by experiment as indicated in main text.
 		Results are mean and std of average accuracy over 3 resp.\ 10 runs for MNIST resp.\ CIFAR. 
 	}
 	\label{table:results}
 	\vskip -0.6in
 	\begin{center}
 		\vskip -0.15in
 		\begin{small}
 			%\vskip -0.1in
 			\begin{sc}
 				%\vskip -0.1in
 				\begin{tabular}{cccc|c|cccc}
 					\toprule
 					\textbf{No.} & \textbf{Algo.} & \textbf{P-MNIST} & \textbf{CIFAR} & &\textbf{No.} & \textbf{Algo.} & \textbf{P-MNIST} & \textbf{CIFAR} \\
 					\midrule
 					\multirow{3}*{(1)}
 					&  $\MAS$ & 97.3$\pm$0.1& 73.7$\pm$0.5 & &\multirow{3}*{(3)} & $\SI$ & 97.2$\pm$0.1& 74.4$\pm$0.5\\
 					& $\MASX$ & 97.4$\pm$0.2& 73.7$\pm$0.2 &
 					&& $\OnAF$& 97.3$\pm$0.1&    74.4$\pm$0.6 \\ 
 					& $\AF$ & 97.4$\pm$0.1& 73.4$\pm$0.4&
 					&& $\AF$ & 97.4$\pm$0.1& 73.4$\pm$0.4\\ 
 					\midrule
 					\multirow{3}*{(2)}
 					& $\SI$ & 97.2$\pm$0.1& 74.4$\pm$0.5& 
 					&\multirow{3}*{(4)} 
 					& Fisher ($\EWC$) & 97.1$\pm$0.3 & 73.1$\pm$0.7 \\
 					& $\SIU$ & 96.3$\pm$0.1& 72.5$\pm$0.8& 
 					&&   Emp. Fisher (EF) & 97.1$\pm$0.1& 73.0$\pm$0.5   \\
 					& $\SIB$ & 97.2$\pm$0.1& 75.1$\pm$0.4&
 					&& Batch-EF & 97.1$\pm$0.1& 73.0$\pm$0.8 \\
 					\bottomrule
 				\end{tabular}
 			\end{sc}
 		\end{small}
 	\end{center}
 	%\vskip -0.1in
 \end{table}
 
 
 
 
 
 
 
 \begin{figure}[t]
 	%\vskip -40pt
 	\begin{center}
 	\begin{subfigure}{0.32\textwidth}
 			\centerline{\includegraphics[width=\textwidth]{../figures/correlations_MAS_cifar.png}}
 			%\vskip 1in
 			\centerline{\includegraphics[width=\textwidth]{../figures/correlations_MAS_mnist.png}}
 	\end{subfigure}
  	\begin{subfigure}{0.32\textwidth}
 		\centerline{\includegraphics[width=\textwidth]{../figures/MAS_MASX_scatter_CIFAR_task_1.png}}
 	\end{subfigure}
   	\begin{subfigure}{0.32\textwidth}
 		\centerline{\includegraphics[width=\textwidth]{../figures/MAS_AF_scatter_CIFAR_task_1.png}}
 	\end{subfigure}
 \end{center}
\vskip -16pt
 	\caption{
 		\textbf{Empirical Relation between MAS, MASX, Absolute Fisher.} \textit{Left}: Summary of Pearson Correlations (top: CIFAR, bottom: MNIST), error bars represent std over 4 runs. \textit{Mid}\&\textit{Right}: Example scatter plots of importance measures. Each point in the scatter plot corresponds to one weight of the net. A straight line through the origin corresponds to two importance measures being multiples of each other. 
 		}
 	\label{figure:MAS}
 	\vskip -0.2in
 \end{figure}
 
 
 
 
 
 
 

